The dependence of the estimated luminosities of ULX on spectral models

Data from {\it Chandra} observations of thirty nearby galaxies were analyzed and 365 X-ray point sources were chosen whose spectra were not contaminated by excessive diffuse emission and not affected by photon pile up. The spectra of these sources were fitted using two spectral models (an absorbed power-law and a disk blackbody) to ascertain the dependence of estimated parameters on the spectral model used. It was found that the cumulative luminosity function depends on the choice of the spectral model, especially for luminosities $> 10^{40}$ ergs/s. In accordance with previous results, a large number ($\sim 80$) of the sources have luminosities $> 10^{39}$ ergs/s (Ultra-Luminous X-ray sources) with indistinguishable average spectral parameters (inner disk temperature $\sim 1$ keV and/or photon index $\Gamma \sim 2$) with those of the lower luminosities ones. After considering foreground stars and known background AGN,we identify four sources whose minimum luminosity exceed $10^{40}$ ergs/s, and call them Extremely Luminous X-ray sources (ELX). The spectra of these sources are in general better represented by the disk black body model than the power-law one. These ELX can be grouped into two distinct spectral classes. Two of them have an inner disk temperature of $< 0.5$ keV and hence are called ``supersoft'' ELX, while the other two have temperatures $\gtrsim 1.3$ keV and are called ``hard'' ELX. The estimated inner disk temperatures of the supersoft ELX are compatible with the hypothesis that they harbor intermediate size black holes, which are accreting at $\sim 0.5$ times their Eddington Luminosity. The radiative mechanism for hard ELX, seems to be Inverse Comptonization, which in contrast to standard black holes systems, is probably saturated.

==> tab4.tex <==

%\LongTables
\begin{deluxetable} {lccccccr}
\tablenum{4}
\tablewidth{0pc}
\tablecaption{
Spectral Properties of point sources fitted with the Power-Law model}
\tablehead{
\colhead{Galaxy} & \colhead{R.A.} & \colhead{Decl.} & \colhead{$n_H$($10^{22}cm^{-2}$)} & \colhead{$\Gamma$} &  \colhead{log(L) ergs/s} & \colhead{C$_{stat}$} & \colhead{d. o. f.}}
\startdata
NGC0253 &   0 47 43.07 & -25 15 29.28 & $ 0.15^{+ 0.53}_{- 0.15}$ & $ 2.52^{+2.31}_{-1.21}$ & $37.70^{+1.20}_{-0.18}$ & $  9.43$ & $   4$ \\
NGC0253 &   0 47 42.80 & -25 15  2.02 & $ 0.77^{+ 0.51}_{- 0.49}$ & $ 1.86^{+0.66}_{-0.77}$ & $38.26^{+0.27}_{-0.12}$ & $  3.36$ & $   4$ \\
NGC0253 &   0 47 35.25 & -25 15 11.53 & $ 0.48^{+ 0.05}_{- 0.13}$ & $ 2.19^{+0.22}_{-0.33}$ & $38.65^{+0.05}_{-0.08}$ & $ 38.94$ & $  19$ \\
NGC0253 &   0 47 34.28 & -25 17  3.32 & $ 5.66^{+ 5.98}_{- 5.66}$ & $ 5.38^{+4.62}_{-4.95}$ & $40.82^{+3.28}_{-2.90}$ & $  3.21$ & $   2$ \\
NGC0253 &   0 47 34.00 & -25 16 36.51 & $ 1.04^{+ 0.11}_{- 0.10}$ & $ 2.19^{+0.22}_{-0.22}$ & $39.01^{+0.08}_{-0.07}$ & $ 10.93$ & $  27$ \\
NGC0253 &   0 47 33.55 & -25 18 16.51 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.64^{+0.99}_{-0.44}$ & $37.33^{+0.15}_{-0.10}$ & $  2.37$ & $   2$ \\
NGC0253 &   0 47 32.05 & -25 17 21.43 & $ 3.17^{+ 2.20}_{- 2.46}$ & $ 1.97^{+1.10}_{-1.10}$ & $38.61^{+0.72}_{-0.32}$ & $  1.63$ & $   3$ \\
NGC0253 &   0 47 30.98 & -25 18 26.23 & $ 1.55^{+ 1.46}_{- 1.55}$ & $ 1.75^{+1.21}_{-1.21}$ & $38.24^{+0.65}_{-0.21}$ & $  1.76$ & $   3$ \\
NGC0253 &   0 47 28.01 & -25 18 20.21 & $ 0.93^{+ 1.13}_{- 0.92}$ & $ 2.08^{+1.76}_{-1.54}$ & $38.02^{+1.03}_{-0.23}$ & $  2.13$ & $   1$ \\
NGC0253 &   0 47 25.20 & -25 19 45.22 & $ 0.00^{+ 0.15}_{- 0.00}$ & $ 1.31^{+0.66}_{-0.22}$ & $37.96^{+0.09}_{-0.09}$ & $  5.10$ & $   4$ \\
NGC0253 &   0 47 18.50 & -25 19 13.94 & $ 0.00^{+ 0.15}_{- 0.00}$ & $ 1.31^{+0.44}_{-0.22}$ & $37.97^{+0.07}_{-0.05}$ & $  3.94$ & $   5$ \\
NGC0253 &   0 47 40.66 & -25 14 11.71 & $ 0.69^{+ 0.72}_{- 0.56}$ & $ 2.41^{+1.98}_{-1.32}$ & $37.96^{+1.11}_{-0.27}$ & $  1.07$ & $   3$ \\
NGC0253 &   0 47 17.65 & -25 18 26.45 & $ 0.11^{+ 0.49}_{- 0.11}$ & $ 1.31^{+1.54}_{-0.77}$ & $38.12^{+0.27}_{-0.12}$ & $  3.13$ & $   3$ \\
NGC0628 &   1 36 51.06 & +15 45 46.86 & $ 0.03^{+ 0.05}_{- 0.03}$ & $ 1.86^{+0.22}_{-0.11}$ & $39.22^{+0.04}_{-0.02}$ & $ 50.58$ & $  36$ \\
NGC0628 &   1 36 47.45 & +15 47 45.01 & $ 0.89^{+ 0.11}_{- 0.33}$ & $ 9.56^{+0.44}_{-2.42}$ & $42.18^{+0.36}_{-1.49}$ & $  8.56$ & $   4$ \\
NGC0628 &   1 36 44.12 & +15 48 18.85 & $ 0.50^{+ 0.21}_{- 0.22}$ & $ 2.30^{+0.55}_{-0.44}$ & $39.09^{+0.22}_{-0.15}$ & $  8.73$ & $   9$ \\
NGC0628 &   1 36 41.73 & +15 47  1.23 & $ 0.09^{+ 0.26}_{- 0.09}$ & $ 1.75^{+0.99}_{-0.66}$ & $38.17^{+0.26}_{-0.25}$ & $  4.96$ & $   3$ \\
NGC0628 &   1 36 41.66 & +15 45 52.30 & $ 0.29^{+ 0.37}_{- 0.28}$ & $ 1.86^{+0.88}_{-0.66}$ & $38.65^{+0.30}_{-0.14}$ & $ 16.79$ & $   3$ \\
NGC0628 &   1 36 39.10 & +15 43  9.86 & $ 0.14^{+ 0.17}_{- 0.14}$ & $ 1.86^{+0.44}_{-0.33}$ & $38.73^{+0.11}_{-0.11}$ & $  2.53$ & $   6$ \\
NGC0628 &   1 36 25.13 & +15 48 59.87 & $ 1.02^{+ 1.26}_{- 1.02}$ & $ 3.51^{+2.53}_{-2.09}$ & $39.37^{+1.93}_{-0.88}$ & $  0.44$ & $   1$ \\
NGC0891 &   2 22 37.08 & +42 21 58.24 & $ 0.48^{+ 0.20}_{- 0.27}$ & $ 1.97^{+0.55}_{-0.55}$ & $38.92^{+0.17}_{-0.09}$ & $  5.92$ & $   7$ \\
NGC0891 &   2 22 35.74 & +42 20 52.91 & $ 0.88^{+ 0.52}_{- 0.49}$ & $ 2.52^{+1.10}_{-0.88}$ & $38.91^{+0.63}_{-0.28}$ & $  0.90$ & $   2$ \\
NGC0891 &   2 22 34.40 & +42 21  0.39 & $ 0.07^{+ 0.20}_{- 0.07}$ & $ 1.75^{+0.55}_{-0.33}$ & $38.65^{+0.13}_{-0.06}$ & $  4.86$ & $   5$ \\
NGC0891 &   2 22 31.91 & +42 22 34.68 & $ 0.03^{+ 0.43}_{- 0.03}$ & $ 1.09^{+0.99}_{-0.44}$ & $38.20^{+0.14}_{-0.14}$ & $  3.88$ & $   2$ \\
NGC0891 &   2 22 31.35 & +42 20 24.33 & $ 0.70^{+ 0.00}_{- 0.00}$ & $ 1.86^{+0.00}_{-0.00}$ & $39.97^{+0.00}_{-0.00}$ & $ 88.06$ & $  83$ \\
NGC0891 &   2 22 31.26 & +42 19 57.79 & $ 0.52^{+ 0.06}_{- 0.06}$ & $ 2.19^{+0.11}_{-0.11}$ & $39.82^{+0.04}_{-0.04}$ & $ 99.52$ & $  62$ \\
NGC0891 &   2 22 28.98 & +42 20 22.22 & $ 0.12^{+ 0.55}_{- 0.12}$ & $ 1.20^{+0.99}_{-0.44}$ & $38.55^{+0.16}_{-0.10}$ & $  3.48$ & $   2$ \\
NGC0891 &   2 22 27.58 & +42 21  8.84 & $ 0.00^{+ 0.12}_{- 0.00}$ & $ 1.64^{+0.44}_{-0.22}$ & $38.50^{+0.07}_{-0.04}$ & $  4.98$ & $   6$ \\
NGC0891 &   2 22 26.28 & +42 18 33.69 & $ 0.00^{+ 0.03}_{- 0.00}$ & $ 1.64^{+0.55}_{-0.44}$ & $38.25^{+0.11}_{-0.09}$ & $  7.52$ & $   4$ \\
NGC0891 &   2 22 25.26 & +42 24 51.64 & $ 0.09^{+ 0.04}_{- 0.03}$ & $ 1.86^{+0.11}_{-0.11}$ & $39.35^{+0.03}_{-0.01}$ & $ 30.52$ & $  43$ \\
NGC0891 &   2 22 24.36 & +42 21 38.98 & $ 0.10^{+ 0.06}_{- 0.04}$ & $ 1.97^{+0.22}_{-0.11}$ & $39.10^{+0.05}_{-0.03}$ & $ 26.00$ & $  24$ \\
NGC0891 &   2 22 15.11 & +42 20 45.01 & $ 0.00^{+ 0.03}_{- 0.00}$ & $ 1.64^{+0.11}_{-0.11}$ & $38.87^{+0.04}_{-0.03}$ & $ 13.49$ & $  16$ \\
NGC0891 &   2 22 15.04 & +42 23 41.75 & $ 0.16^{+ 0.20}_{- 0.16}$ & $ 2.08^{+0.77}_{-0.55}$ & $38.52^{+0.25}_{-0.14}$ & $  6.51$ & $   3$ \\
NGC0891 &   2 22 42.13 & +42 24  3.02 & $ 0.10^{+ 0.23}_{- 0.10}$ & $ 1.09^{+0.66}_{-0.44}$ & $38.77^{+0.11}_{-0.09}$ & $  1.16$ & $   5$ \\
NGC1291 &   3 17 26.34 & -41  5 44.53 & $ 0.00^{+ 0.08}_{- 0.00}$ & $ 1.86^{+0.55}_{-0.33}$ & $38.06^{+0.12}_{-0.08}$ & $  4.44$ & $   4$ \\
NGC1291 &   3 17 23.45 & -41  6 49.13 & $ 0.00^{+ 0.41}_{- 0.00}$ & $ 1.09^{+2.31}_{-0.55}$ & $38.32^{+0.29}_{-0.22}$ & $  1.41$ & $   1$ \\
NGC1291 &   3 17 21.69 & -41  6 52.34 & $ 0.09^{+ 0.22}_{- 0.09}$ & $ 1.42^{+0.77}_{-0.55}$ & $38.43^{+0.11}_{-0.10}$ & $  2.47$ & $   2$ \\
NGC1291 &   3 17 21.43 & -41  7 34.42 & $ 0.00^{+ 0.15}_{- 0.00}$ & $ 1.20^{+0.55}_{-0.22}$ & $38.28^{+0.07}_{-0.09}$ & $  2.70$ & $   4$ \\
NGC1291 &   3 17 19.35 & -41  6 14.92 & $ 0.03^{+ 0.17}_{- 0.03}$ & $ 1.31^{+0.55}_{-0.33}$ & $38.46^{+0.08}_{-0.10}$ & $  7.89$ & $   3$ \\
NGC1291 &   3 17 17.50 & -41  7 18.72 & $ 0.00^{+ 0.26}_{- 0.00}$ & $ 2.19^{+2.09}_{-0.44}$ & $37.87^{+0.73}_{-0.10}$ & $  1.62$ & $   1$ \\
NGC1291 &   3 17 16.66 & -41  5 13.36 & $ 0.20^{+ 0.18}_{- 0.16}$ & $ 3.84^{+1.32}_{-1.21}$ & $38.69^{+0.70}_{-0.48}$ & $  2.17$ & $   3$ \\
NGC1291 &   3 17 16.51 & -41  7 13.22 & $ 0.00^{+ 0.13}_{- 0.00}$ & $ 1.42^{+0.55}_{-0.33}$ & $37.98^{+0.13}_{-0.37}$ & $  0.60$ & $   2$ \\
NGC1291 &   3 17 14.98 & -41  6 12.37 & $ 0.01^{+ 0.17}_{- 0.01}$ & $ 0.98^{+0.77}_{-0.33}$ & $38.61^{+0.13}_{-0.13}$ & $  3.71$ & $   3$ \\
NGC1291 &   3 17 13.81 & -41  7 26.55 & $ 0.00^{+ 0.24}_{- 0.00}$ & $ 1.20^{+0.99}_{-0.33}$ & $38.46^{+0.14}_{-0.13}$ & $  0.99$ & $   2$ \\
NGC1291 &   3 17  8.85 & -41  5 34.19 & $ 0.77^{+ 1.63}_{- 0.77}$ & $ 2.74^{+3.85}_{-2.42}$ & $38.55^{+2.73}_{-0.47}$ & $  0.66$ & $   1$ \\
NGC1291 &   3 17  2.53 & -41  7 13.98 & $ 0.17^{+ 0.07}_{- 0.07}$ & $ 2.52^{+0.33}_{-0.44}$ & $39.14^{+0.11}_{-0.08}$ & $ 26.65$ & $  23$ \\
NGC1291 &   3 17 23.83 & -41  9 50.75 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 1.42^{+1.76}_{-0.66}$ & $38.16^{+0.32}_{-0.19}$ & $  2.06$ & $   2$ \\
NGC1291 &   3 17 22.36 & -41  9 25.62 & $ 0.00^{+ 0.29}_{- 0.00}$ & $ 0.65^{+0.66}_{-0.33}$ & $38.53^{+0.13}_{-0.14}$ & $  5.18$ & $   2$ \\
NGC1316 &   3 22 51.23 & -37  9 49.43 & $ 0.39^{+ 0.14}_{- 0.15}$ & $ 4.39^{+0.99}_{-0.99}$ & $40.21^{+0.55}_{-0.50}$ & $  9.36$ & $   9$ \\
NGC1316 &   3 22 42.68 & -37 12 17.11 & $ 0.58^{+ 0.66}_{- 0.58}$ & $ 4.39^{+3.19}_{-2.53}$ & $39.79^{+2.12}_{-1.11}$ & $  1.46$ & $   2$ \\
NGC1316 &   3 22 42.46 & -37 12 21.56 & $ 0.00^{+ 0.21}_{- 0.00}$ & $ 2.08^{+1.10}_{-0.55}$ & $38.84^{+0.33}_{-0.02}$ & $  1.84$ & $   2$ \\
NGC1316 &   3 22 42.09 & -37 11 23.18 & $ 0.03^{+ 0.43}_{- 0.03}$ & $ 1.53^{+1.10}_{-0.44}$ & $38.85^{+0.28}_{-0.09}$ & $  0.46$ & $   1$ \\
NGC1316 &   3 22 40.77 & -37 12 23.94 & $ 0.00^{+ 0.08}_{- 0.00}$ & $ 1.64^{+0.44}_{-0.22}$ & $38.91^{+0.07}_{-0.09}$ & $  7.99$ & $   3$ \\
NGC1316 &   3 22 40.50 & -37 12 26.71 & $ 0.25^{+ 0.46}_{- 0.25}$ & $ 4.28^{+3.41}_{-1.87}$ & $39.29^{+1.97}_{-0.76}$ & $  3.96$ & $   3$ \\
NGC1316 &   3 22 36.43 & -37 13 23.75 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.86^{+1.21}_{-0.66}$ & $38.80^{+0.23}_{-0.08}$ & $  2.10$ & $   1$ \\
NGC1316 &   3 22 35.55 & -37 13 13.17 & $ 0.00^{+ 0.23}_{- 0.00}$ & $ 2.08^{+1.32}_{-0.44}$ & $38.78^{+0.40}_{-0.07}$ & $  4.17$ & $   2$ \\
NGC1316 &   3 22 25.70 & -37  9 12.36 & $ 0.05^{+ 0.14}_{- 0.05}$ & $ 2.63^{+0.88}_{-0.44}$ & $39.08^{+0.36}_{-0.11}$ & $  0.71$ & $   4$ \\
NGC1399 &   3 38 51.61 & -35 26 43.59 & $ 0.05^{+ 0.01}_{- 0.03}$ & $ 1.64^{+0.11}_{-0.11}$ & $39.82^{+0.02}_{-0.02}$ & $ 57.11$ & $  48$ \\
NGC1399 &   3 38 48.71 & -35 28 34.34 & $ 0.01^{+ 0.07}_{- 0.01}$ & $ 2.19^{+0.55}_{-0.22}$ & $38.97^{+0.09}_{-0.06}$ & $ 13.02$ & $   9$ \\
NGC1399 &   3 38 45.35 & -35 27 37.07 & $ 0.29^{+ 0.15}_{- 0.17}$ & $ 2.19^{+0.55}_{-0.55}$ & $39.09^{+0.20}_{-0.11}$ & $  3.83$ & $   4$ \\
NGC1399 &   3 38 44.96 & -35 28 21.50 & $ 0.01^{+ 0.24}_{- 0.01}$ & $ 1.42^{+1.32}_{-0.55}$ & $38.50^{+0.22}_{-0.15}$ & $  0.98$ & $   2$ \\
NGC1399 &   3 38 41.37 & -35 31 34.06 & $ 0.00^{+ 0.01}_{- 0.00}$ & $ 1.82^{+0.07}_{-0.05}$ & $40.24^{+0.01}_{-0.00}$ & $140.56$ & $  98$ \\
NGC1399 &   3 38 38.80 & -35 25 54.39 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.53^{+0.99}_{-0.33}$ & $38.60^{+0.12}_{-0.12}$ & $  0.10$ & $   2$ \\
NGC1399 &   3 38 38.62 & -35 27 27.58 & $ 0.19^{+ 0.42}_{- 0.19}$ & $ 2.08^{+1.87}_{-1.32}$ & $38.53^{+0.78}_{-0.19}$ & $  3.21$ & $   2$ \\
NGC1399 &   3 38 36.83 & -35 27 46.75 & $ 0.00^{+ 0.16}_{- 0.00}$ & $ 2.19^{+1.21}_{-0.22}$ & $38.73^{+0.31}_{-0.05}$ & $ 11.25$ & $   4$ \\
NGC1399 &   3 38 36.34 & -35 27  8.40 & $ 0.00^{+ 0.22}_{- 0.00}$ & $ 1.97^{+0.99}_{-0.44}$ & $38.43^{+0.32}_{-0.06}$ & $  1.61$ & $   3$ \\
NGC1399 &   3 38 36.30 & -35 28  9.19 & $ 0.00^{+ 0.47}_{- 0.00}$ & $ 1.09^{+0.66}_{-0.44}$ & $38.72^{+0.12}_{-0.07}$ & $  3.27$ & $   2$ \\
NGC1399 &   3 38 36.17 & -35 26 25.11 & $ 0.00^{+ 0.39}_{- 0.00}$ & $ 1.75^{+2.97}_{-0.55}$ & $38.30^{+0.95}_{-0.19}$ & $  0.78$ & $   2$ \\
NGC1399 &   3 38 33.82 & -35 25 56.43 & $ 0.06^{+ 0.29}_{- 0.06}$ & $ 2.19^{+1.65}_{-0.66}$ & $38.55^{+0.65}_{-0.12}$ & $  1.68$ & $   2$ \\
NGC1399 &   3 38 33.80 & -35 26 57.96 & $ 0.18^{+ 0.25}_{- 0.18}$ & $ 2.41^{+1.32}_{-0.99}$ & $38.54^{+0.61}_{-0.20}$ & $  1.36$ & $   3$ \\
NGC1399 &   3 38 33.18 & -35 25 53.26 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 1.42^{+1.21}_{-0.66}$ & $38.44^{+0.26}_{-0.17}$ & $  1.69$ & $   2$ \\
NGC1399 &   3 38 33.12 & -35 27 31.29 & $ 0.01^{+ 0.04}_{- 0.01}$ & $ 1.75^{+0.22}_{-0.22}$ & $38.91^{+0.06}_{-0.04}$ & $  9.36$ & $   7$ \\
NGC1399 &   3 38 32.80 & -35 26 58.29 & $ 0.09^{+ 0.22}_{- 0.09}$ & $ 1.53^{+1.10}_{-0.66}$ & $38.84^{+0.17}_{-0.12}$ & $  0.11$ & $   2$ \\
NGC1399 &   3 38 32.60 & -35 27  5.12 & $ 0.02^{+ 0.04}_{- 0.02}$ & $ 1.42^{+0.22}_{-0.11}$ & $39.55^{+0.04}_{-0.03}$ & $ 18.80$ & $  26$ \\
NGC1399 &   3 38 32.35 & -35 27  1.75 & $ 0.47^{+ 0.57}_{- 0.30}$ & $ 2.63^{+1.54}_{-1.10}$ & $38.95^{+0.86}_{-0.26}$ & $  4.67$ & $   2$ \\
NGC1399 &   3 38 32.33 & -35 26 45.73 & $ 0.09^{+ 0.22}_{- 0.09}$ & $ 4.17^{+2.64}_{-1.54}$ & $38.54^{+1.13}_{-0.41}$ & $  0.02$ & $   1$ \\
NGC1399 &   3 38 32.34 & -35 27 10.34 & $ 0.19^{+ 0.43}_{- 0.19}$ & $ 1.86^{+1.54}_{-0.99}$ & $38.80^{+0.56}_{-0.14}$ & $  0.15$ & $   1$ \\
NGC1399 &   3 38 31.90 & -35 26 49.04 & $ 0.00^{+ 0.07}_{- 0.00}$ & $ 2.41^{+0.77}_{-0.22}$ & $38.64^{+0.13}_{-0.11}$ & $  3.53$ & $   3$ \\
NGC1399 &   3 38 31.82 & -35 26  3.76 & $ 0.09^{+ 0.05}_{- 0.04}$ & $ 2.85^{+0.44}_{-0.33}$ & $39.35^{+0.15}_{-0.07}$ & $ 25.55$ & $  19$ \\
NGC1399 &   3 38 31.73 & -35 30 58.65 & $ 0.01^{+ 0.16}_{- 0.01}$ & $ 2.52^{+1.65}_{-0.55}$ & $38.56^{+0.50}_{-0.11}$ & $  5.68$ & $   2$ \\
NGC1399 &   3 38 29.84 & -35 27 48.02 & $ 0.01^{+ 0.15}_{- 0.01}$ & $ 1.20^{+0.66}_{-0.33}$ & $38.54^{+0.11}_{-0.10}$ & $  3.02$ & $   3$ \\
NGC1399 &   3 38 29.68 & -35 25  4.10 & $ 0.05^{+ 0.16}_{- 0.05}$ & $ 1.64^{+1.10}_{-0.55}$ & $38.97^{+0.15}_{-0.09}$ & $ 10.68$ & $   5$ \\
NGC1399 &   3 38 27.76 & -35 27 50.20 & $ 0.00^{+ 0.29}_{- 0.00}$ & $ 0.76^{+0.77}_{-0.66}$ & $38.94^{+0.22}_{-0.19}$ & $  4.31$ & $   2$ \\
NGC1399 &   3 38 27.64 & -35 26 48.16 & $ 0.14^{+ 0.06}_{- 0.07}$ & $ 2.85^{+0.44}_{-0.44}$ & $39.42^{+0.16}_{-0.14}$ & $ 32.22$ & $  19$ \\
NGC1399 &   3 38 27.17 & -35 26  0.91 & $ 0.01^{+ 0.40}_{- 0.01}$ & $ 1.53^{+2.09}_{-0.66}$ & $38.64^{+0.54}_{-0.15}$ & $  6.96$ & $   1$ \\
NGC1399 &   3 38 26.50 & -35 27 31.91 & $ 0.16^{+ 0.30}_{- 0.16}$ & $ 2.30^{+1.54}_{-1.10}$ & $38.88^{+0.65}_{-0.14}$ & $  0.56$ & $   2$ \\
NGC1399 &   3 38 25.94 & -35 27 41.77 & $ 0.00^{+ 0.16}_{- 0.00}$ & $ 1.75^{+0.66}_{-0.44}$ & $38.62^{+0.12}_{-0.09}$ & $  1.43$ & $   2$ \\
NGC1399 &   3 38 25.28 & -35 27 52.97 & $ 0.03^{+ 0.26}_{- 0.03}$ & $ 1.42^{+0.88}_{-0.44}$ & $38.57^{+0.15}_{-0.14}$ & $  3.68$ & $   4$ \\
NGC1399 &   3 38 25.29 & -35 25 21.92 & $ 0.00^{+ 0.02}_{- 0.00}$ & $ 1.97^{+0.11}_{-0.22}$ & $38.93^{+0.06}_{-0.03}$ & $  8.54$ & $   9$ \\
NGC1399 &   3 38 21.91 & -35 29 28.30 & $ 0.05^{+ 0.13}_{- 0.05}$ & $ 1.42^{+0.55}_{-0.33}$ & $39.02^{+0.10}_{-0.10}$ & $ 15.65$ & $   5$ \\
NGC1399 &   3 38 31.68 & -35 26  0.22 & $ 0.07^{+ 0.18}_{- 0.07}$ & $ 1.97^{+0.99}_{-0.66}$ & $38.52^{+0.27}_{-0.13}$ & $  0.99$ & $   4$ \\
NGC1399 &   3 38 28.96 & -35 26  2.00 & $ 0.01^{+ 0.17}_{- 0.01}$ & $ 1.31^{+0.66}_{-0.33}$ & $38.65^{+0.10}_{-0.09}$ & $  0.65$ & $   4$ \\
NGC1399 &   3 38 25.62 & -35 25 55.34 & $ 0.49^{+ 0.80}_{- 0.49}$ & $ 3.18^{+2.97}_{-1.98}$ & $38.90^{+1.94}_{-0.57}$ & $  0.10$ & $   1$ \\
NGC1569 &   4 31 25.17 & +64 51 54.10 & $ 6.11^{+ 1.58}_{- 1.79}$ & $ 1.42^{+0.55}_{-0.66}$ & $38.20^{+0.22}_{-0.15}$ & $  5.63$ & $  15$ \\
NGC1569 &   4 31 20.52 & +64 51 22.51 & $ 0.26^{+ 0.26}_{- 0.26}$ & $ 1.53^{+0.55}_{-0.55}$ & $37.21^{+0.10}_{-0.06}$ & $  2.07$ & $   6$ \\
NGC1569 &   4 31 14.56 & +64 50 24.52 & $ 0.82^{+ 1.48}_{- 0.82}$ & $ 2.08^{+1.43}_{-0.99}$ & $37.00^{+0.92}_{-0.26}$ & $  2.26$ & $   3$ \\
NGC1569 &   4 31 14.02 & +64 51  7.94 & $ 0.43^{+ 0.11}_{- 0.05}$ & $ 5.38^{+0.77}_{-0.33}$ & $38.77^{+0.46}_{-0.19}$ & $116.74$ & $  29$ \\
NGC1569 &   4 31 13.21 & +64 52 29.54 & $ 0.25^{+ 0.10}_{- 0.07}$ & $ 2.08^{+0.33}_{-0.22}$ & $37.49^{+0.10}_{-0.05}$ & $ 10.97$ & $  17$ \\
NGC1569 &   4 30 58.37 & +64 48 52.37 & $ 1.03^{+ 0.60}_{- 0.67}$ & $ 7.36^{+2.64}_{-3.74}$ & $39.31^{+1.92}_{-2.31}$ & $  4.78$ & $   2$ \\
NGC1569 &   4 30 57.42 & +64 50 48.62 & $ 0.81^{+ 0.33}_{- 0.35}$ & $ 2.41^{+0.44}_{-0.66}$ & $37.60^{+0.26}_{-0.19}$ & $  8.79$ & $   9$ \\
NGC1569 &   4 30 49.86 & +64 50 55.48 & $ 0.00^{+ 0.13}_{- 0.00}$ & $ 1.20^{+0.33}_{-0.22}$ & $37.14^{+0.05}_{-0.06}$ & $  9.42$ & $   7$ \\
NGC1569 &   4 30 48.62 & +64 50 58.59 & $ 0.24^{+ 0.06}_{- 0.05}$ & $ 1.64^{+0.22}_{-0.11}$ & $37.72^{+0.03}_{-0.02}$ & $ 36.90$ & $  33$ \\
NGC1569 &   4 30 48.26 & +64 50 46.65 & $ 0.38^{+ 0.38}_{- 0.27}$ & $ 1.42^{+0.55}_{-0.44}$ & $37.29^{+0.13}_{-0.05}$ & $ 16.03$ & $   7$ \\
NGC1569 &   4 30 48.14 & +64 50 50.57 & $ 0.51^{+ 0.06}_{- 0.06}$ & $ 4.06^{+0.33}_{-0.22}$ & $38.66^{+0.19}_{-0.15}$ & $ 88.44$ & $  50$ \\
NGC1569 &   4 30 34.33 & +64 47 40.56 & $ 0.43^{+ 0.05}_{- 0.13}$ & $ 2.08^{+0.22}_{-0.22}$ & $37.62^{+0.04}_{-0.07}$ & $ 17.01$ & $  18$ \\
NGC1569 &   4 30 30.88 & +64 52  5.38 & $ 0.09^{+ 0.19}_{- 0.09}$ & $ 1.42^{+0.44}_{-0.33}$ & $37.14^{+0.07}_{-0.05}$ & $  5.44$ & $   7$ \\
NGC1569 &   4 30 25.27 & +64 50 35.72 & $ 1.09^{+ 1.64}_{- 1.09}$ & $ 2.96^{+2.53}_{-1.87}$ & $37.38^{+1.96}_{-0.57}$ & $  1.66$ & $   1$ \\
NGC1569 &   4 31 24.43 & +64 51 15.89 & $ 0.69^{+ 0.54}_{- 0.69}$ & $ 2.30^{+1.10}_{-1.10}$ & $36.91^{+0.59}_{-0.30}$ & $  1.70$ & $   3$ \\
NGC2403 &   7 37 14.94 & +65 34 28.83 & $ 0.41^{+ 0.88}_{- 0.41}$ & $ 1.75^{+2.09}_{-1.32}$ & $37.58^{+0.95}_{-0.17}$ & $  1.23$ & $   1$ \\
NGC2403 &   7 37 11.63 & +65 33 45.52 & $ 0.63^{+ 0.26}_{- 0.18}$ & $ 2.30^{+0.44}_{-0.33}$ & $38.39^{+0.21}_{-0.12}$ & $ 21.83$ & $  13$ \\
NGC2403 &   7 36 42.03 & +65 36 51.99 & $ 0.95^{+ 0.12}_{- 0.10}$ & $ 9.67^{+0.33}_{-0.88}$ & $41.54^{+0.33}_{-0.51}$ & $ 23.54$ & $   7$ \\
NGC2403 &   7 36 32.91 & +65 34 58.01 & $ 0.33^{+ 0.60}_{- 0.33}$ & $ 3.40^{+3.96}_{-2.64}$ & $37.67^{+2.26}_{-0.54}$ & $  2.11$ & $   2$ \\
NGC3034 &   9 56 19.57 & +69 41 45.50 & $ 0.75^{+ 0.58}_{- 0.64}$ & $ 1.97^{+0.88}_{-0.77}$ & $38.30^{+0.40}_{-0.17}$ & $  0.81$ & $   3$ \\
NGC3034 &   9 55 54.55 & +69 41  0.39 & $ 4.24^{+ 1.75}_{- 1.56}$ & $ 2.63^{+0.88}_{-0.77}$ & $39.48^{+0.71}_{-0.45}$ & $  8.52$ & $  13$ \\
NGC3034 &   9 55 37.94 & +69 40 28.87 & $ 0.41^{+ 0.62}_{- 0.41}$ & $ 2.08^{+0.99}_{-0.77}$ & $38.08^{+0.50}_{-0.21}$ & $  1.02$ & $   2$ \\
NGC3034 &   9 55 27.00 & +69 39 23.15 & $ 0.31^{+ 0.38}_{- 0.29}$ & $ 1.97^{+0.55}_{-0.44}$ & $38.33^{+0.23}_{-0.12}$ & $  5.59$ & $   7$ \\
NGC3034 &   9 55 20.70 & +69 44 42.97 & $ 0.19^{+ 0.58}_{- 0.19}$ & $ 2.52^{+1.32}_{-0.77}$ & $38.02^{+0.76}_{-0.17}$ & $  1.78$ & $   3$ \\
NGC3079 &  10  2  5.39 & +55 42 58.29 & $ 0.55^{+ 0.68}_{- 0.55}$ & $ 1.31^{+0.66}_{-0.55}$ & $39.58^{+0.18}_{-0.09}$ & $  2.46$ & $   4$ \\
NGC3079 &  10  2  2.88 & +55 38 58.82 & $ 0.04^{+ 0.10}_{- 0.04}$ & $ 1.20^{+0.33}_{-0.22}$ & $39.62^{+0.06}_{-0.05}$ & $  6.45$ & $  12$ \\
NGC3079 &  10  1 58.11 & +55 41  3.65 & $ 0.04^{+ 0.47}_{- 0.04}$ & $ 1.86^{+1.65}_{-0.66}$ & $38.84^{+0.58}_{-0.07}$ & $  1.01$ & $   3$ \\
NGC3079 &  10  1 52.11 & +55 39  5.24 & $ 0.00^{+ 0.06}_{- 0.00}$ & $ 1.64^{+0.55}_{-0.33}$ & $38.84^{+0.09}_{-0.09}$ & $  2.77$ & $   2$ \\
NGC3079 &  10  2  1.01 & +55 36 48.20 & $ 0.00^{+ 0.04}_{- 0.00}$ & $ 1.97^{+0.44}_{-0.33}$ & $39.11^{+0.07}_{-0.03}$ & $  5.30$ & $   3$ \\
NGC3379 &  10 47 52.78 & +12 35  8.46 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.64^{+0.88}_{-0.22}$ & $38.42^{+0.13}_{-0.10}$ & $  3.09$ & $   2$ \\
NGC3379 &  10 47 52.66 & +12 33 37.77 & $ 0.16^{+ 0.20}_{- 0.16}$ & $ 2.08^{+0.88}_{-0.88}$ & $38.92^{+0.27}_{-0.13}$ & $  3.57$ & $   4$ \\
NGC3379 &  10 47 49.11 & +12 34 48.72 & $ 0.06^{+ 0.15}_{- 0.06}$ & $ 1.64^{+0.66}_{-0.44}$ & $38.86^{+0.08}_{-0.09}$ & $  6.81$ & $   5$ \\
NGC3379 &  10 47 47.98 & +12 34 45.69 & $ 1.24^{+ 0.15}_{- 0.68}$ & $ 9.67^{+0.33}_{-4.18}$ & $42.49^{+0.32}_{-2.72}$ & $  1.66$ & $   2$ \\
NGC3379 &  10 47 46.96 & +12 34 38.61 & $ 0.06^{+ 0.12}_{- 0.06}$ & $ 2.41^{+0.88}_{-0.55}$ & $38.71^{+0.28}_{-0.12}$ & $  2.65$ & $   5$ \\
NGC3379 &  10 47 46.82 & +12 34 27.23 & $ 0.53^{+ 0.66}_{- 0.53}$ & $ 2.74^{+2.09}_{-1.54}$ & $38.83^{+1.26}_{-0.39}$ & $  0.57$ & $   1$ \\
NGC3379 &  10 47 41.85 & +12 37 45.36 & $ 0.71^{+ 0.42}_{- 0.36}$ & $ 7.14^{+2.86}_{-2.53}$ & $41.14^{+1.79}_{-1.47}$ & $ 17.03$ & $   4$ \\
NGC3556 &  11 11 48.99 & +55 40 24.45 & $ 0.25^{+ 0.55}_{- 0.25}$ & $ 2.41^{+2.20}_{-1.54}$ & $38.47^{+1.16}_{-0.23}$ & $  0.72$ & $   2$ \\
NGC3556 &  11 11 41.41 & +55 40 57.74 & $ 0.97^{+ 0.76}_{- 0.93}$ & $ 1.97^{+0.88}_{-0.88}$ & $39.43^{+0.42}_{-0.22}$ & $  4.38$ & $   7$ \\
NGC3556 &  11 11 40.50 & +55 40 12.83 & $ 0.38^{+ 0.57}_{- 0.38}$ & $ 2.63^{+1.54}_{-1.21}$ & $38.95^{+0.89}_{-0.30}$ & $  1.93$ & $   2$ \\
NGC3556 &  11 11 39.02 & +55 41  2.58 & $ 0.69^{+ 0.40}_{- 0.69}$ & $ 7.91^{+2.09}_{-4.73}$ & $41.36^{+1.44}_{-2.61}$ & $  0.36$ & $   3$ \\
NGC3556 &  11 11 38.39 & +55 39 51.79 & $ 0.00^{+ 0.15}_{- 0.00}$ & $ 1.53^{+0.33}_{-0.33}$ & $38.61^{+0.11}_{-0.05}$ & $  1.44$ & $   2$ \\
NGC3556 &  11 11 38.21 & +55 42 36.84 & $ 0.97^{+ 0.75}_{- 0.69}$ & $ 1.31^{+0.55}_{-0.55}$ & $39.34^{+0.16}_{-0.08}$ & $ 11.98$ & $   8$ \\
NGC3556 &  11 11 38.15 & +55 40 19.23 & $ 0.17^{+ 0.31}_{- 0.17}$ & $ 2.30^{+1.32}_{-0.88}$ & $38.88^{+0.55}_{-0.12}$ & $  2.56$ & $   4$ \\
NGC3556 &  11 11 35.26 & +55 41  7.28 & $ 0.04^{+ 0.63}_{- 0.04}$ & $ 1.09^{+1.98}_{-0.66}$ & $38.74^{+0.35}_{-0.16}$ & $  0.58$ & $   2$ \\
NGC3556 &  11 11 30.34 & +55 40 31.29 & $ 0.33^{+ 0.19}_{- 0.18}$ & $ 1.86^{+0.22}_{-0.33}$ & $39.33^{+0.10}_{-0.09}$ & $ 12.40$ & $  12$ \\
NGC3556 &  11 11 26.90 & +55 39 14.83 & $ 0.07^{+ 0.09}_{- 0.07}$ & $ 1.97^{+0.33}_{-0.33}$ & $38.91^{+0.09}_{-0.06}$ & $  3.08$ & $   8$ \\
NGC3556 &  11 11 26.82 & +55 40 28.78 & $ 0.16^{+ 0.35}_{- 0.16}$ & $ 2.08^{+0.99}_{-0.77}$ & $38.65^{+0.39}_{-0.12}$ & $  0.73$ & $   3$ \\
NGC3556 &  11 11 26.05 & +55 40 16.79 & $ 0.33^{+ 0.04}_{- 0.04}$ & $ 1.86^{+0.11}_{-0.11}$ & $39.84^{+0.02}_{-0.02}$ & $ 60.26$ & $  54$ \\
NGC3556 &  11 11 17.71 & +55 40  9.83 & $ 0.12^{+ 0.12}_{- 0.11}$ & $ 2.08^{+0.44}_{-0.44}$ & $38.99^{+0.12}_{-0.08}$ & $  5.66$ & $   9$ \\
NGC3556 &  11 11 25.74 & +55 44  1.58 & $ 0.01^{+ 0.05}_{- 0.01}$ & $ 1.97^{+0.22}_{-0.22}$ & $39.06^{+0.06}_{-0.06}$ & $ 19.23$ & $  15$ \\
NGC3556 &  11 11 17.87 & +55 40 17.08 & $ 0.02^{+ 0.07}_{- 0.02}$ & $ 0.76^{+0.33}_{-0.33}$ & $38.99^{+0.08}_{-0.09}$ & $  1.76$ & $   3$ \\
NGC3628 &  11 20 26.72 & +13 34 58.22 & $ 0.00^{+ 0.34}_{- 0.00}$ & $ 1.42^{+0.66}_{-0.33}$ & $38.04^{+0.15}_{-0.07}$ & $  2.84$ & $   2$ \\
NGC3628 &  11 20 24.38 & +13 38 22.94 & $ 0.10^{+ 0.35}_{- 0.10}$ & $ 1.75^{+0.55}_{-0.33}$ & $38.75^{+0.15}_{-0.06}$ & $  6.30$ & $   6$ \\
NGC3628 &  11 20 20.72 & +13 35  7.57 & $ 3.25^{+ 2.93}_{- 2.74}$ & $ 2.85^{+1.98}_{-1.76}$ & $39.50^{+1.72}_{-0.76}$ & $  1.84$ & $   3$ \\
NGC3628 &  11 20 16.25 & +13 35 27.20 & $ 1.07^{+ 0.76}_{- 0.87}$ & $ 1.75^{+0.66}_{-0.77}$ & $39.01^{+0.29}_{-0.14}$ & $  0.69$ & $   6$ \\
NGC3628 &  11 20 15.80 & +13 37 47.67 & $ 0.04^{+ 0.13}_{- 0.04}$ & $ 1.75^{+0.55}_{-0.33}$ & $38.53^{+0.10}_{-0.09}$ & $ 19.27$ & $   4$ \\
NGC3628 &  11 20 14.72 & +13 32 27.71 & $ 0.02^{+ 0.02}_{- 0.02}$ & $ 1.97^{+0.11}_{-0.11}$ & $38.93^{+0.02}_{-0.03}$ & $ 21.43$ & $  27$ \\
NGC3628 &  11 20 13.61 & +13 34 40.95 & $ 0.62^{+ 0.68}_{- 0.61}$ & $ 1.31^{+0.99}_{-0.88}$ & $38.83^{+0.24}_{-0.08}$ & $  6.18$ & $   4$ \\
NGC3628 &  11 20 13.35 & +13 35  8.52 & $ 0.46^{+ 0.78}_{- 0.46}$ & $ 1.09^{+0.88}_{-0.77}$ & $38.35^{+0.20}_{-0.12}$ & $  2.45$ & $   3$ \\
NGC3628 &  11 20 11.21 & +13 34 45.79 & $ 0.00^{+ 0.55}_{- 0.00}$ & $ 1.42^{+2.42}_{-0.77}$ & $38.23^{+0.68}_{-0.16}$ & $  1.13$ & $   1$ \\
NGC3628 &  11 20 10.41 & +13 39 34.14 & $ 0.00^{+ 0.02}_{- 0.00}$ & $ 1.64^{+0.00}_{-0.11}$ & $39.35^{+0.02}_{-0.00}$ & $ 43.53$ & $  40$ \\
NGC3628 &  11 20  9.66 & +13 37 13.09 & $ 0.29^{+ 0.80}_{- 0.29}$ & $ 1.75^{+1.43}_{-0.88}$ & $38.42^{+0.61}_{-0.18}$ & $  6.05$ & $   2$ \\
NGC3628 &  11 20  6.94 & +13 34 54.56 & $ 0.00^{+ 0.07}_{- 0.00}$ & $ 1.64^{+0.22}_{-0.22}$ & $38.33^{+0.07}_{-0.08}$ & $  6.59$ & $   3$ \\
NGC3628 &  11 20 33.50 & +13 35 25.42 & $ 0.00^{+ 0.30}_{- 0.00}$ & $ 0.87^{+0.66}_{-0.33}$ & $38.33^{+0.10}_{-0.13}$ & $  2.13$ & $   3$ \\
NGC3628 &  11 20 11.82 & +13 31 22.55 & $ 0.00^{+ 0.01}_{- 0.00}$ & $ 1.97^{+0.00}_{-0.11}$ & $38.93^{+0.03}_{-0.00}$ & $ 36.39$ & $  27$ \\
NGC4125 &  12  8 17.91 & +65 11 19.37 & $ 0.54^{+ 0.52}_{- 0.40}$ & $ 3.40^{+2.09}_{-1.54}$ & $39.42^{+1.33}_{-0.56}$ & $  0.11$ & $   1$ \\
NGC4125 &  12  8 17.45 & +65 11 25.28 & $ 0.01^{+ 0.34}_{- 0.01}$ & $ 1.09^{+0.66}_{-0.22}$ & $39.14^{+0.07}_{-0.08}$ & $  1.77$ & $   2$ \\
NGC4125 &  12  8  7.53 & +65 10 28.46 & $ 0.03^{+ 0.02}_{- 0.03}$ & $ 1.97^{+0.11}_{-0.11}$ & $39.91^{+0.02}_{-0.02}$ & $ 33.02$ & $  42$ \\
NGC4125 &  12  8  7.26 & +65 11 49.05 & $ 0.00^{+ 0.06}_{- 0.00}$ & $ 1.75^{+0.33}_{-0.22}$ & $39.04^{+0.06}_{-0.05}$ & $  2.30$ & $   4$ \\
NGC4125 &  12  8  1.73 & +65 10 34.66 & $ 0.00^{+ 0.29}_{- 0.00}$ & $ 1.53^{+0.88}_{-0.55}$ & $38.93^{+0.16}_{-0.06}$ & $  2.50$ & $   2$ \\
NGC4125 &  12  7 56.90 & +65  7 15.90 & $ 0.05^{+ 0.27}_{- 0.05}$ & $ 2.41^{+1.65}_{-0.66}$ & $38.91^{+0.66}_{-0.11}$ & $  0.64$ & $   3$ \\
NGC4125 &  12  7 35.74 & +65 10 22.69 & $ 0.00^{+ 0.14}_{- 0.00}$ & $ 1.75^{+0.88}_{-0.33}$ & $39.10^{+0.11}_{-0.07}$ & $  2.46$ & $   4$ \\
NGC4125 &  12  8 11.51 & +65  6 10.03 & $ 0.00^{+ 0.45}_{- 0.00}$ & $ 1.53^{+2.42}_{-0.66}$ & $38.97^{+0.67}_{-0.15}$ & $  6.43$ & $   1$ \\
NGC4365 &  12 24 29.72 & + 7 19  4.07 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 0.76^{+0.99}_{-0.55}$ & $39.01^{+0.27}_{-0.19}$ & $  2.12$ & $   2$ \\
NGC4365 &  12 24 28.50 & + 7 18 31.09 & $ 0.00^{+ 0.39}_{- 0.00}$ & $ 2.08^{+2.53}_{-0.55}$ & $38.84^{+0.96}_{-0.07}$ & $  0.89$ & $   1$ \\
NGC4365 &  12 24 27.74 & + 7 18  6.87 & $ 0.80^{+ 0.33}_{- 0.80}$ & $ 8.13^{+1.87}_{-5.94}$ & $41.68^{+1.29}_{-3.00}$ & $  0.32$ & $   2$ \\
NGC4365 &  12 24 26.39 & + 7 16 53.18 & $ 0.19^{+ 0.48}_{- 0.19}$ & $ 1.31^{+0.55}_{-0.44}$ & $39.51^{+0.12}_{-0.10}$ & $  3.65$ & $   5$ \\
NGC4365 &  12 24 25.68 & + 7 17 46.01 & $ 0.78^{+ 0.60}_{- 0.50}$ & $ 5.60^{+3.19}_{-2.53}$ & $40.53^{+2.16}_{-1.46}$ & $  2.92$ & $   2$ \\
NGC4365 &  12 24 20.18 & + 7 17 39.42 & $ 0.01^{+ 0.05}_{- 0.01}$ & $ 1.53^{+0.88}_{-0.66}$ & $38.87^{+0.22}_{-0.13}$ & $  0.80$ & $   2$ \\
NGC4365 &  12 24 14.75 & + 7 20  4.77 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 2.30^{+1.21}_{-0.33}$ & $39.02^{+0.41}_{-0.02}$ & $  1.09$ & $   3$ \\
NGC4365 &  12 24 38.29 & + 7 21  7.01 & $ 0.26^{+ 0.32}_{- 0.26}$ & $ 4.06^{+2.09}_{-1.65}$ & $39.52^{+1.25}_{-0.63}$ & $  1.64$ & $   3$ \\
NGC4365 &  12 24 14.61 & + 7 15 35.15 & $ 0.00^{+ 0.11}_{- 0.00}$ & $ 1.97^{+0.22}_{-0.33}$ & $39.26^{+0.09}_{-0.02}$ & $  8.44$ & $   3$ \\
NGC4374 &  12 25 15.09 & +12 56  2.70 & $ 0.01^{+ 0.03}_{- 0.01}$ & $ 1.86^{+0.22}_{-0.22}$ & $39.48^{+0.04}_{-0.03}$ & $  7.54$ & $  15$ \\
NGC4374 &  12 25  5.38 & +12 53 45.39 & $ 0.00^{+ 0.29}_{- 0.00}$ & $ 1.64^{+1.43}_{-0.55}$ & $38.75^{+0.33}_{-0.08}$ & $  3.44$ & $   2$ \\
NGC4374 &  12 25  1.58 & +12 52 35.93 & $ 0.49^{+ 0.61}_{- 0.49}$ & $ 4.06^{+2.97}_{-2.20}$ & $39.60^{+1.93}_{-0.91}$ & $  0.29$ & $   2$ \\
NGC4374 &  12 24 46.91 & +12 54 35.00 & $ 0.25^{+ 0.46}_{- 0.25}$ & $ 3.18^{+2.86}_{-1.98}$ & $39.40^{+1.59}_{-0.38}$ & $  2.28$ & $   3$ \\
NGC4449 &  12 28 13.26 & +44  6 55.82 & $ 0.16^{+ 0.19}_{- 0.16}$ & $ 2.41^{+0.99}_{-0.99}$ & $38.18^{+0.36}_{-0.12}$ & $  5.22$ & $   7$ \\
NGC4449 &  12 28 11.98 & +44  6 41.46 & $ 0.22^{+ 0.28}_{- 0.22}$ & $ 2.96^{+1.54}_{-1.21}$ & $38.15^{+0.77}_{-0.31}$ & $  7.19$ & $   4$ \\
NGC4449 &  12 28 11.19 & +44  6 38.52 & $ 0.49^{+ 0.38}_{- 0.32}$ & $ 4.83^{+2.42}_{-1.76}$ & $38.78^{+1.50}_{-0.96}$ & $  0.64$ & $   1$ \\
NGC4449 &  12 28 10.95 & +44  6 48.48 & $ 0.31^{+ 0.04}_{- 0.06}$ & $ 3.07^{+0.22}_{-0.22}$ & $39.04^{+0.10}_{-0.12}$ & $107.79$ & $  36$ \\
NGC4449 &  12 28 10.93 & +44  3 37.99 & $ 0.17^{+ 0.07}_{- 0.05}$ & $ 6.15^{+0.99}_{-0.88}$ & $39.03^{+0.42}_{-0.29}$ & $ 23.11$ & $  12$ \\
NGC4449 &  12 28  9.71 & +44  5 53.11 & $ 0.15^{+ 0.28}_{- 0.15}$ & $ 1.31^{+0.77}_{-0.55}$ & $38.17^{+0.10}_{-0.07}$ & $  3.32$ & $   5$ \\
NGC4449 &  12 28  9.31 & +44  5  8.27 & $ 0.16^{+ 0.04}_{- 0.03}$ & $ 2.74^{+0.22}_{-0.11}$ & $38.83^{+0.09}_{-0.06}$ & $ 74.79$ & $  43$ \\
NGC4449 &  12 28  7.34 & +44  4 53.79 & $ 0.32^{+ 0.49}_{- 0.32}$ & $ 4.83^{+3.41}_{-2.42}$ & $38.66^{+2.05}_{-1.04}$ & $  3.71$ & $   3$ \\
NGC4449 &  12 28  7.28 & +44  7 21.57 & $ 0.13^{+ 0.46}_{- 0.13}$ & $ 1.42^{+1.10}_{-0.66}$ & $37.68^{+0.26}_{-0.12}$ & $  0.10$ & $   1$ \\
NGC4449 &  12 28  3.88 & +44  5 43.84 & $ 0.00^{+ 0.28}_{- 0.00}$ & $ 1.42^{+0.99}_{-0.33}$ & $37.81^{+0.16}_{-0.08}$ & $  0.97$ & $   2$ \\
NGC4449 &  12 28  2.07 & +44  8  7.95 & $ 0.68^{+ 0.53}_{- 0.46}$ & $ 3.51^{+1.98}_{-1.76}$ & $38.56^{+1.28}_{-0.61}$ & $  4.40$ & $   2$ \\
NGC4485 &  12 30 49.60 & +41 40 56.74 & $ 0.00^{+ 0.09}_{- 0.00}$ & $ 1.86^{+0.22}_{-0.22}$ & $38.92^{+0.06}_{-0.01}$ & $  5.50$ & $   7$ \\
NGC4485 &  12 30 40.42 & +41 38 13.42 & $ 0.62^{+ 0.61}_{- 0.62}$ & $ 1.86^{+0.99}_{-0.99}$ & $38.84^{+0.41}_{-0.15}$ & $  0.56$ & $   3$ \\
NGC4485 &  12 30 36.33 & +41 38 37.78 & $ 0.38^{+ 0.16}_{- 0.11}$ & $ 1.75^{+0.22}_{-0.22}$ & $39.47^{+0.07}_{-0.03}$ & $ 24.77$ & $  22$ \\
NGC4485 &  12 30 34.45 & +41 38 49.86 & $ 0.55^{+ 0.68}_{- 0.55}$ & $ 2.52^{+1.43}_{-1.21}$ & $39.00^{+0.85}_{-0.31}$ & $  1.12$ & $   2$ \\
NGC4485 &  12 30 32.27 & +41 39 18.07 & $ 0.39^{+ 0.10}_{- 0.11}$ & $ 1.75^{+0.22}_{-0.22}$ & $39.47^{+0.04}_{-0.04}$ & $ 16.54$ & $  21$ \\
NGC4485 &  12 30 30.82 & +41 39 11.48 & $ 0.83^{+ 0.10}_{- 0.17}$ & $ 1.86^{+0.22}_{-0.22}$ & $39.73^{+0.06}_{-0.06}$ & $ 20.73$ & $  29$ \\
NGC4485 &  12 30 30.40 & +41 38 52.86 & $ 0.37^{+ 0.55}_{- 0.37}$ & $ 1.64^{+0.66}_{-0.55}$ & $38.92^{+0.24}_{-0.11}$ & $  2.66$ & $   4$ \\
NGC4485 &  12 30 29.55 & +41 39 27.61 & $ 3.16^{+ 0.82}_{- 0.65}$ & $ 3.73^{+0.77}_{-0.55}$ & $40.65^{+0.68}_{-0.46}$ & $  8.66$ & $  10$ \\
NGC4485 &  12 30 25.30 & +41 39 24.74 & $ 0.26^{+ 0.89}_{- 0.26}$ & $ 1.64^{+1.54}_{-0.88}$ & $38.48^{+0.65}_{-0.14}$ & $  3.39$ & $   2$ \\
NGC4559 &  12 35 57.79 & +27 58  7.43 & $ 0.29^{+ 0.17}_{- 0.16}$ & $ 2.08^{+0.55}_{-0.55}$ & $39.54^{+0.17}_{-0.09}$ & $ 12.45$ & $   7$ \\
NGC4579 &  12 37 53.89 & +11 50 20.33 & $ 0.08^{+ 0.18}_{- 0.08}$ & $ 1.64^{+0.88}_{-0.55}$ & $39.30^{+0.12}_{-0.10}$ & $  2.46$ & $   3$ \\
NGC4579 &  12 37 44.13 & +11 49 17.32 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 1.31^{+0.44}_{-0.33}$ & $38.97^{+0.08}_{-0.07}$ & $  1.94$ & $   3$ \\
NGC4579 &  12 37 40.30 & +11 47 27.48 & $ 0.15^{+ 0.02}_{- 0.03}$ & $ 1.75^{+0.11}_{-0.11}$ & $40.37^{+0.00}_{-0.02}$ & $ 74.52$ & $  63$ \\
NGC4594 &  12 40  7.06 & -11 37 53.49 & $ 0.00^{+ 0.55}_{- 0.00}$ & $ 1.31^{+1.32}_{-0.66}$ & $38.47^{+0.29}_{-0.12}$ & $  3.05$ & $   1$ \\
NGC4594 &  12 40  2.01 & -11 39 40.56 & $ 0.53^{+ 0.44}_{- 0.47}$ & $ 7.69^{+2.31}_{-4.73}$ & $40.67^{+1.83}_{-2.06}$ & $  1.96$ & $   2$ \\
NGC4594 &  12 40  1.09 & -11 37 24.13 & $ 0.34^{+ 0.12}_{- 0.09}$ & $ 5.05^{+0.88}_{-0.66}$ & $40.26^{+0.51}_{-0.36}$ & $ 23.76$ & $  17$ \\
NGC4594 &  12 40  0.97 & -11 36 54.20 & $ 0.14^{+ 0.11}_{- 0.13}$ & $ 2.19^{+0.55}_{-0.66}$ & $39.18^{+0.15}_{-0.07}$ & $  5.34$ & $   9$ \\
NGC4594 &  12 40  0.71 & -11 35 19.74 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 1.20^{+0.55}_{-0.22}$ & $38.73^{+0.07}_{-0.10}$ & $  0.42$ & $   2$ \\
NGC4594 &  12 40  0.38 & -11 37 23.70 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.97^{+1.10}_{-0.55}$ & $38.55^{+0.26}_{-0.05}$ & $  1.47$ & $   2$ \\
NGC4594 &  12 40  0.07 & -11 37  8.75 & $ 0.47^{+ 0.64}_{- 0.46}$ & $ 2.52^{+1.54}_{-1.10}$ & $38.86^{+0.92}_{-0.58}$ & $  0.09$ & $   1$ \\
NGC4594 &  12 39 59.93 & -11 36 23.27 & $ 0.00^{+ 0.49}_{- 0.00}$ & $ 0.98^{+1.54}_{-0.55}$ & $38.86^{+0.23}_{-0.41}$ & $  7.41$ & $   1$ \\
NGC4594 &  12 39 59.10 & -11 37 19.78 & $ 0.39^{+ 0.76}_{- 0.39}$ & $ 4.61^{+4.73}_{-2.86}$ & $39.49^{+2.98}_{-1.03}$ & $  0.05$ & $   1$ \\
NGC4594 &  12 39 57.41 & -11 37 20.07 & $ 0.00^{+ 0.13}_{- 0.00}$ & $ 1.09^{+0.44}_{-0.33}$ & $38.90^{+0.12}_{-0.12}$ & $  7.64$ & $   2$ \\
NGC4594 &  12 39 51.98 & -11 35 52.18 & $ 0.00^{+ 0.55}_{- 0.00}$ & $ 2.30^{+3.08}_{-1.10}$ & $38.49^{+1.46}_{-0.02}$ & $  1.77$ & $   1$ \\
NGC4594 &  12 39 50.96 & -11 38 23.63 & $ 1.14^{+ 0.82}_{- 0.72}$ & $ 3.18^{+1.54}_{-1.21}$ & $39.50^{+1.13}_{-0.59}$ & $  0.10$ & $   1$ \\
NGC4594 &  12 39 48.62 & -11 37 13.33 & $ 0.08^{+ 0.16}_{- 0.08}$ & $ 2.08^{+0.66}_{-0.55}$ & $38.89^{+0.20}_{-0.09}$ & $  4.35$ & $   4$ \\
NGC4594 &  12 39 45.22 & -11 38 49.81 & $ 0.54^{+ 0.12}_{- 0.10}$ & $ 5.93^{+0.77}_{-0.77}$ & $41.16^{+0.48}_{-0.43}$ & $125.51$ & $  26$ \\
NGC4594 &  12 40 10.46 & -11 36 39.07 & $ 0.00^{+ 0.21}_{- 0.00}$ & $ 1.42^{+0.55}_{-0.33}$ & $38.70^{+0.10}_{-0.38}$ & $  4.82$ & $   2$ \\
NGC4594 &  12 39 59.04 & -11 35 12.01 & $ 0.63^{+ 0.49}_{- 0.45}$ & $ 2.52^{+1.10}_{-1.10}$ & $39.06^{+0.63}_{-0.30}$ & $  1.14$ & $   2$ \\
NGC4594 &  12 39 45.27 & -11 36  0.63 & $ 0.28^{+ 0.37}_{- 0.28}$ & $ 1.97^{+0.99}_{-0.88}$ & $38.82^{+0.38}_{-0.16}$ & $  1.88$ & $   2$ \\
NGC4594 &  12 39 43.63 & -11 40 34.08 & $ 0.14^{+ 0.39}_{- 0.14}$ & $ 2.19^{+0.99}_{-0.66}$ & $38.93^{+0.44}_{-0.10}$ & $  7.58$ & $   3$ \\
NGC4631 &  12 42 11.13 & +32 32 35.94 & $ 4.02^{+ 0.49}_{- 0.44}$ & $ 2.74^{+0.33}_{-0.22}$ & $40.28^{+0.25}_{-0.16}$ & $ 47.60$ & $  48$ \\
NGC4631 &  12 42  7.37 & +32 32 33.82 & $ 0.82^{+ 0.82}_{- 0.79}$ & $ 1.97^{+0.88}_{-0.77}$ & $38.78^{+0.45}_{-0.21}$ & $  3.70$ & $   5$ \\
NGC4631 &  12 42  6.61 & +32 32  8.44 & $ 2.70^{+ 2.68}_{- 2.56}$ & $ 3.29^{+2.75}_{-2.42}$ & $39.20^{+2.39}_{-1.00}$ & $  0.44$ & $   1$ \\
NGC4631 &  12 42  6.18 & +32 31 53.08 & $ 0.51^{+ 1.77}_{- 0.51}$ & $ 0.98^{+2.09}_{-1.10}$ & $38.04^{+0.75}_{-0.16}$ & $  1.82$ & $   1$ \\
NGC4631 &  12 42  6.13 & +32 32 46.64 & $ 0.28^{+ 0.22}_{- 0.15}$ & $ 1.53^{+0.44}_{-0.33}$ & $38.76^{+0.09}_{-0.06}$ & $ 24.06$ & $  13$ \\
NGC4631 &  12 42  5.48 & +32 30 37.39 & $ 0.34^{+ 0.62}_{- 0.34}$ & $ 2.74^{+2.86}_{-2.09}$ & $37.91^{+1.62}_{-0.35}$ & $  0.02$ & $   1$ \\
NGC4631 &  12 42  5.00 & +32 31 52.15 & $ 1.44^{+ 1.43}_{- 1.40}$ & $ 1.97^{+1.65}_{-1.54}$ & $38.38^{+0.96}_{-0.27}$ & $  6.02$ & $   1$ \\
NGC4631 &  12 42  4.04 & +32 34  8.51 & $ 0.00^{+ 0.72}_{- 0.00}$ & $ 0.76^{+2.42}_{-0.55}$ & $38.45^{+0.30}_{-0.25}$ & $  1.33$ & $   1$ \\
NGC4631 &  12 42  0.11 & +32 31 58.99 & $ 0.08^{+ 0.08}_{- 0.08}$ & $ 1.97^{+0.44}_{-0.44}$ & $38.42^{+0.08}_{-0.05}$ & $ 10.23$ & $  12$ \\
NGC4631 &  12 41 58.02 & +32 28 51.28 & $ 0.08^{+ 0.04}_{- 0.03}$ & $ 1.64^{+0.22}_{-0.11}$ & $38.94^{+0.02}_{-0.02}$ & $ 38.07$ & $  36$ \\
NGC4631 &  12 41 57.41 & +32 32  3.11 & $ 0.39^{+ 0.83}_{- 0.39}$ & $ 3.73^{+4.07}_{-2.53}$ & $38.44^{+2.60}_{-0.72}$ & $  8.81$ & $   1$ \\
NGC4631 &  12 41 55.98 & +32 30 44.88 & $ 0.00^{+ 5.95}_{- 0.00}$ & $ 0.65^{+2.64}_{-0.66}$ & $38.38^{+1.25}_{-0.06}$ & $  0.39$ & $   1$ \\
NGC4649 &  12 43 48.62 & +11 32 40.96 & $ 0.00^{+ 0.49}_{- 0.00}$ & $ 2.08^{+3.41}_{-0.66}$ & $38.51^{+1.41}_{-0.07}$ & $  0.04$ & $   2$ \\
NGC4649 &  12 43 47.03 & +11 32 36.75 & $ 0.00^{+ 0.13}_{- 0.00}$ & $ 1.31^{+0.44}_{-0.11}$ & $39.08^{+0.06}_{-0.04}$ & $  2.00$ & $   4$ \\
NGC4649 &  12 43 46.91 & +11 32 33.85 & $ 0.00^{+ 0.21}_{- 0.00}$ & $ 1.53^{+1.32}_{-0.55}$ & $38.66^{+0.24}_{-0.20}$ & $  1.31$ & $   1$ \\
NGC4649 &  12 43 45.00 & +11 32 33.33 & $ 0.00^{+ 0.13}_{- 0.00}$ & $ 1.53^{+0.55}_{-0.33}$ & $39.01^{+0.09}_{-0.08}$ & $  4.52$ & $   3$ \\
NGC4649 &  12 43 44.56 & +11 31 50.74 & $ 0.05^{+ 0.44}_{- 0.05}$ & $ 1.31^{+1.21}_{-0.55}$ & $38.85^{+0.20}_{-0.14}$ & $  9.35$ & $   1$ \\
NGC4649 &  12 43 43.59 & +11 33  2.66 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.97^{+0.99}_{-0.44}$ & $38.59^{+0.26}_{-0.08}$ & $  3.30$ & $   2$ \\
NGC4649 &  12 43 41.77 & +11 34 33.78 & $ 0.00^{+ 0.26}_{- 0.00}$ & $ 1.86^{+1.87}_{-0.44}$ & $38.91^{+0.47}_{-0.11}$ & $  0.77$ & $   2$ \\
NGC4649 &  12 43 40.46 & +11 32 43.01 & $ 0.00^{+ 0.13}_{- 0.00}$ & $ 1.86^{+0.77}_{-0.44}$ & $38.85^{+0.14}_{-0.06}$ & $  2.87$ & $   2$ \\
NGC4649 &  12 43 38.07 & +11 32 41.74 & $ 0.06^{+ 0.37}_{- 0.06}$ & $ 1.20^{+1.76}_{-0.77}$ & $38.68^{+0.28}_{-0.18}$ & $  0.01$ & $   2$ \\
NGC4649 &  12 43 37.94 & +11 34 35.22 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 1.31^{+0.88}_{-0.44}$ & $38.64^{+0.16}_{-0.10}$ & $  3.22$ & $   2$ \\
NGC4649 &  12 43 37.84 & +11 33 28.36 & $ 0.12^{+ 0.25}_{- 0.12}$ & $ 1.86^{+0.88}_{-0.66}$ & $38.69^{+0.27}_{-0.13}$ & $  1.61$ & $   3$ \\
NGC4649 &  12 43 37.27 & +11 31 43.68 & $ 0.00^{+ 0.03}_{- 0.00}$ & $ 1.86^{+0.22}_{-0.11}$ & $39.07^{+0.03}_{-0.05}$ & $  7.38$ & $   8$ \\
NGC4649 &  12 43 36.49 & +11 30  8.96 & $ 0.00^{+ 0.03}_{- 0.00}$ & $ 2.52^{+0.11}_{-0.22}$ & $39.98^{+0.05}_{-0.00}$ & $ 12.52$ & $  13$ \\
NGC4649 &  12 43 35.48 & +11 34 27.30 & $ 0.01^{+ 0.43}_{- 0.01}$ & $ 1.53^{+2.20}_{-0.55}$ & $38.78^{+0.60}_{-0.20}$ & $  8.23$ & $   1$ \\
NGC4649 &  12 43 34.79 & +11 32 27.49 & $ 0.14^{+ 0.29}_{- 0.14}$ & $ 2.30^{+0.99}_{-0.77}$ & $38.77^{+0.44}_{-0.21}$ & $  7.92$ & $   3$ \\
NGC4649 &  12 43 34.04 & +11 33 41.88 & $ 0.05^{+ 0.19}_{- 0.05}$ & $ 1.53^{+0.77}_{-0.44}$ & $39.04^{+0.10}_{-0.11}$ & $  1.46$ & $   3$ \\
NGC4649 &  12 43 33.94 & +11 34  1.24 & $ 0.00^{+ 0.40}_{- 0.00}$ & $ 0.98^{+1.98}_{-0.55}$ & $38.89^{+0.27}_{-0.27}$ & $  0.89$ & $   2$ \\
NGC4649 &  12 43 33.30 & +11 32 39.86 & $ 0.00^{+ 0.18}_{- 0.00}$ & $ 1.09^{+0.55}_{-0.33}$ & $39.01^{+0.12}_{-0.11}$ & $  1.24$ & $   3$ \\
NGC4649 &  12 43 32.64 & +11 30  2.04 & $ 0.09^{+ 0.32}_{- 0.09}$ & $ 2.08^{+0.99}_{-0.55}$ & $39.07^{+0.38}_{-0.09}$ & $  3.81$ & $   2$ \\
NGC4649 &  12 43 32.08 & +11 34 18.57 & $ 0.00^{+ 1.06}_{- 0.00}$ & $ 1.09^{+1.43}_{-0.44}$ & $39.14^{+0.35}_{-0.13}$ & $  0.60$ & $   2$ \\
NGC4649 &  12 43 32.03 & +11 31 46.64 & $ 0.00^{+ 0.06}_{- 0.00}$ & $ 1.86^{+0.44}_{-0.55}$ & $38.71^{+0.12}_{-0.08}$ & $  7.14$ & $   2$ \\
NGC4649 &  12 43 29.87 & +11 33 18.25 & $ 0.00^{+ 0.29}_{- 0.00}$ & $ 1.09^{+0.77}_{-0.44}$ & $38.84^{+0.16}_{-0.15}$ & $  0.92$ & $   1$ \\
NGC4649 &  12 43 55.01 & +11 33  7.98 & $ 0.01^{+ 0.24}_{- 0.01}$ & $ 1.64^{+1.54}_{-0.44}$ & $38.96^{+0.26}_{-0.13}$ & $  3.80$ & $   3$ \\
NGC4697 &  12 48 47.49 &  -5 45 13.03 & $ 0.00^{+ 0.46}_{- 0.00}$ & $ 1.75^{+1.98}_{-0.77}$ & $38.95^{+0.65}_{-0.07}$ & $  0.40$ & $   1$ \\
NGC4697 &  12 48 46.84 &  -5 48 53.64 & $ 0.00^{+ 0.05}_{- 0.00}$ & $ 1.09^{+0.22}_{-0.11}$ & $39.12^{+0.05}_{-0.09}$ & $ 33.79$ & $  11$ \\
NGC4697 &  12 48 45.44 &  -5 45 42.64 & $ 0.28^{+ 0.56}_{- 0.28}$ & $ 3.95^{+3.63}_{-2.09}$ & $38.96^{+2.17}_{-0.67}$ & $  1.95$ & $   1$ \\
NGC4697 &  12 48 39.36 &  -5 47 30.62 & $ 0.02^{+ 0.36}_{- 0.02}$ & $ 1.42^{+1.76}_{-0.55}$ & $38.34^{+0.33}_{-0.20}$ & $  0.45$ & $   2$ \\
NGC4697 &  12 48 39.31 &  -5 48  7.54 & $ 0.02^{+ 0.14}_{- 0.02}$ & $ 1.42^{+0.66}_{-0.22}$ & $38.81^{+0.08}_{-0.08}$ & $  2.13$ & $   5$ \\
NGC4697 &  12 48 37.50 &  -5 47 43.71 & $ 0.00^{+ 0.28}_{- 0.00}$ & $ 1.53^{+1.76}_{-0.55}$ & $38.24^{+0.32}_{-0.18}$ & $  1.28$ & $   2$ \\
NGC4697 &  12 48 36.96 &  -5 48  1.38 & $ 0.00^{+ 0.26}_{- 0.00}$ & $ 1.31^{+1.54}_{-0.55}$ & $38.34^{+0.29}_{-0.20}$ & $  2.35$ & $   2$ \\
NGC4697 &  12 48 36.71 &  -5 47 32.10 & $ 0.16^{+ 0.31}_{- 0.16}$ & $ 1.53^{+0.99}_{-0.77}$ & $38.73^{+0.19}_{-0.09}$ & $  0.11$ & $   2$ \\
NGC4697 &  12 48 35.97 &  -5 47 56.88 & $ 0.00^{+ 0.25}_{- 0.00}$ & $ 1.42^{+0.77}_{-0.33}$ & $38.37^{+0.11}_{-0.09}$ & $  0.35$ & $   3$ \\
NGC4697 &  12 48 35.92 &  -5 47 52.58 & $ 0.00^{+ 0.38}_{- 0.00}$ & $ 0.87^{+1.43}_{-0.55}$ & $38.52^{+0.28}_{-0.18}$ & $  0.73$ & $   2$ \\
NGC4697 &  12 48 34.53 &  -5 47 49.74 & $ 0.34^{+ 6.38}_{- 0.34}$ & $ 6.26^{+3.74}_{-4.40}$ & $39.50^{+2.92}_{-1.50}$ & $  3.56$ & $   1$ \\
NGC4697 &  12 48 34.49 &  -5 47 40.36 & $ 0.00^{+ 0.17}_{- 0.00}$ & $ 0.76^{+0.66}_{-0.33}$ & $38.59^{+0.14}_{-0.16}$ & $  0.80$ & $   1$ \\
NGC4697 &  12 48 33.19 &  -5 47 42.15 & $ 0.07^{+ 0.10}_{- 0.07}$ & $ 1.53^{+0.44}_{-0.33}$ & $38.84^{+0.06}_{-0.05}$ & $  2.67$ & $   6$ \\
NGC4697 &  12 48 30.81 &  -5 48 37.29 & $ 0.14^{+ 0.28}_{- 0.14}$ & $ 2.08^{+1.43}_{-0.99}$ & $38.49^{+0.50}_{-0.15}$ & $  0.20$ & $   1$ \\
NGC4697 &  12 48 27.33 &  -5 47  8.08 & $ 0.19^{+ 0.43}_{- 0.19}$ & $ 2.08^{+1.65}_{-0.99}$ & $38.62^{+0.68}_{-0.16}$ & $  0.18$ & $   1$ \\
NGC4697 &  12 48 24.44 &  -5 45 58.06 & $ 0.84^{+ 0.18}_{- 0.22}$ & $ 1.75^{+0.22}_{-0.33}$ & $39.63^{+0.09}_{-0.05}$ & $ 26.54$ & $  20$ \\
NGC4697 &  12 48 23.73 &  -5 46 59.79 & $ 0.00^{+ 0.38}_{- 0.00}$ & $ 1.53^{+1.76}_{-0.66}$ & $38.20^{+0.43}_{-0.49}$ & $  1.94$ & $   1$ \\
NGC4697 &  12 48 27.01 &  -5 49 26.02 & $ 0.46^{+ 0.56}_{- 0.46}$ & $ 3.51^{+3.08}_{-2.64}$ & $38.96^{+1.84}_{-0.57}$ & $  0.05$ & $   1$ \\
NGC4697 &  12 48 22.45 &  -5 48 15.38 & $ 0.00^{+ 0.19}_{- 0.00}$ & $ 1.53^{+1.21}_{-0.66}$ & $38.31^{+0.24}_{-0.14}$ & $  1.31$ & $   2$ \\
NGC5055 &  13 16  2.27 & +42  1 53.65 & $ 0.58^{+ 0.07}_{- 0.12}$ & $ 3.51^{+0.33}_{-0.44}$ & $39.99^{+0.18}_{-0.24}$ & $ 24.74$ & $  22$ \\
NGC5055 &  13 15 53.89 & +42  1  4.70 & $ 0.52^{+ 0.64}_{- 0.52}$ & $ 1.75^{+0.77}_{-0.66}$ & $38.91^{+0.33}_{-0.13}$ & $  1.49$ & $   3$ \\
NGC5055 &  13 15 53.25 & +42  2 14.84 & $ 0.09^{+ 0.11}_{- 0.09}$ & $ 1.86^{+0.44}_{-0.33}$ & $38.91^{+0.09}_{-0.08}$ & $ 11.40$ & $   9$ \\
NGC5055 &  13 15 51.39 & +42  1 40.42 & $ 0.19^{+ 0.19}_{- 0.12}$ & $ 4.72^{+1.76}_{-1.32}$ & $39.41^{+0.90}_{-0.50}$ & $  7.79$ & $   7$ \\
NGC5055 &  13 15 50.93 & +42  2  0.17 & $ 0.22^{+ 0.56}_{- 0.22}$ & $ 1.42^{+1.54}_{-1.10}$ & $38.69^{+0.40}_{-0.11}$ & $  0.73$ & $   1$ \\
NGC5055 &  13 15 50.04 & +42  2 15.40 & $ 0.74^{+ 0.74}_{- 0.66}$ & $ 3.62^{+2.86}_{-2.31}$ & $39.18^{+1.89}_{-0.76}$ & $  2.50$ & $   1$ \\
NGC5055 &  13 15 49.57 & +42  1 27.09 & $ 0.00^{+ 1.44}_{- 0.00}$ & $ 0.32^{+0.99}_{-0.33}$ & $39.02^{+0.09}_{-0.09}$ & $  1.19$ & $   2$ \\
NGC5055 &  13 15 49.47 & +41 59 51.75 & $ 0.00^{+ 0.65}_{- 0.00}$ & $ 1.53^{+1.54}_{-0.55}$ & $38.39^{+0.50}_{-0.04}$ & $  3.11$ & $   2$ \\
NGC5055 &  13 15 47.81 & +42  1 24.99 & $ 0.91^{+ 0.71}_{- 0.91}$ & $ 1.75^{+0.88}_{-0.99}$ & $38.83^{+0.37}_{-0.19}$ & $  6.73$ & $   2$ \\
NGC5055 &  13 15 46.64 & +42  2  0.96 & $ 0.98^{+ 0.12}_{- 0.29}$ & $ 9.56^{+0.44}_{-1.98}$ & $42.26^{+0.37}_{-1.24}$ & $  7.62$ & $   4$ \\
NGC5055 &  13 15 43.86 & +41 59 10.34 & $ 0.00^{+ 0.36}_{- 0.00}$ & $ 1.64^{+1.65}_{-0.44}$ & $38.45^{+0.42}_{-0.12}$ & $  1.02$ & $   2$ \\
NGC5055 &  13 15 40.85 & +42  1 49.29 & $ 0.10^{+ 0.10}_{- 0.10}$ & $ 1.75^{+0.44}_{-0.44}$ & $38.92^{+0.06}_{-0.05}$ & $ 10.00$ & $   9$ \\
NGC5055 &  13 15 39.71 & +42  1 10.97 & $ 0.26^{+ 0.20}_{- 0.23}$ & $ 2.52^{+0.77}_{-0.66}$ & $38.96^{+0.33}_{-0.19}$ & $  4.12$ & $   5$ \\
NGC5055 &  13 15 39.49 & +42  2 26.57 & $ 2.43^{+ 1.89}_{- 1.94}$ & $ 3.84^{+2.97}_{-2.64}$ & $39.92^{+2.45}_{-1.26}$ & $  6.15$ & $   2$ \\
NGC5055 &  13 15 39.32 & +42  1 53.38 & $ 0.56^{+ 0.43}_{- 0.49}$ & $ 2.19^{+0.77}_{-0.66}$ & $39.05^{+0.37}_{-0.22}$ & $  2.74$ & $   4$ \\
NGC5055 &  13 15 30.18 & +42  3 13.48 & $ 0.67^{+ 0.17}_{- 0.19}$ & $ 7.25^{+1.32}_{-1.54}$ & $41.36^{+0.75}_{-0.88}$ & $151.54$ & $  11$ \\
NGC5128 &  13 25 58.80 & -43  4 31.27 & $ 0.03^{+ 0.09}_{- 0.03}$ & $ 1.64^{+0.22}_{-0.11}$ & $38.67^{+0.03}_{-0.02}$ & $ 25.69$ & $  29$ \\
NGC5128 &  13 25 44.08 & -43  6 10.97 & $ 0.27^{+ 0.68}_{- 0.27}$ & $ 1.64^{+0.77}_{-0.55}$ & $38.02^{+0.30}_{-0.09}$ & $  5.13$ & $   2$ \\
NGC5128 &  13 25 40.64 & -43  1 15.49 & $ 0.00^{+ 0.11}_{- 0.00}$ & $ 1.20^{+0.88}_{-0.55}$ & $38.00^{+0.20}_{-0.38}$ & $  1.21$ & $   2$ \\
NGC5128 &  13 25 38.38 & -43  2  6.36 & $ 0.82^{+ 0.34}_{- 0.36}$ & $ 1.42^{+0.33}_{-0.44}$ & $38.73^{+0.09}_{-0.05}$ & $ 11.19$ & $  16$ \\
NGC5128 &  13 25 36.71 & -43  0 58.14 & $ 0.09^{+ 0.69}_{- 0.09}$ & $ 1.31^{+0.99}_{-0.44}$ & $37.71^{+0.25}_{-0.07}$ & $  1.96$ & $   3$ \\
NGC5128 &  13 25 33.43 & -43  0 53.11 & $ 0.33^{+ 0.99}_{- 0.33}$ & $ 1.53^{+1.32}_{-0.77}$ & $37.93^{+0.48}_{-0.14}$ & $  1.52$ & $   2$ \\
NGC5128 &  13 25 32.53 & -43  1 34.82 & $ 0.48^{+ 1.23}_{- 0.48}$ & $ 0.76^{+0.88}_{-0.66}$ & $38.25^{+0.15}_{-0.09}$ & $  2.77$ & $   3$ \\
NGC5128 &  13 25 32.09 & -43  2 32.27 & $ 0.01^{+ 0.62}_{- 0.01}$ & $ 1.42^{+0.99}_{-0.33}$ & $37.91^{+0.26}_{-0.06}$ & $  1.20$ & $   3$ \\
NGC5128 &  13 25 31.68 & -43  0  3.65 & $ 0.22^{+ 0.41}_{- 0.22}$ & $ 1.64^{+0.55}_{-0.44}$ & $38.11^{+0.18}_{-0.10}$ & $  8.61$ & $   4$ \\
NGC5128 &  13 25 28.82 & -42 59 48.60 & $ 0.44^{+ 0.35}_{- 0.37}$ & $ 1.86^{+0.66}_{-0.55}$ & $38.25^{+0.22}_{-0.12}$ & $  5.84$ & $   5$ \\
NGC5128 &  13 25 28.28 & -43  2 54.14 & $ 0.13^{+ 0.51}_{- 0.13}$ & $ 2.74^{+1.65}_{-0.77}$ & $37.76^{+0.94}_{-0.20}$ & $  2.38$ & $   3$ \\
NGC5128 &  13 25 27.52 & -43  2 14.78 & $ 0.02^{+ 0.08}_{- 0.02}$ & $ 1.75^{+0.44}_{-0.33}$ & $38.00^{+0.06}_{-0.04}$ & $  3.38$ & $   4$ \\
NGC5128 &  13 25 27.57 & -43  1 28.85 & $ 0.87^{+ 1.07}_{- 0.87}$ & $ 1.64^{+0.99}_{-0.88}$ & $38.25^{+0.44}_{-0.79}$ & $  3.93$ & $   4$ \\
NGC5128 &  13 25 27.15 & -43  1 59.88 & $ 0.37^{+ 0.46}_{- 0.37}$ & $ 1.97^{+0.77}_{-0.77}$ & $38.13^{+0.32}_{-0.16}$ & $  0.26$ & $   3$ \\
NGC5128 &  13 25 25.84 & -43  0 56.39 & $ 0.51^{+ 0.30}_{- 0.33}$ & $ 2.19^{+0.55}_{-0.55}$ & $38.61^{+0.24}_{-0.14}$ & $ 19.97$ & $  12$ \\
NGC5128 &  13 25 24.28 & -42 59 59.89 & $ 0.75^{+ 1.62}_{- 0.75}$ & $ 1.31^{+1.10}_{-0.66}$ & $38.19^{+0.44}_{-0.12}$ & $  5.74$ & $   4$ \\
NGC5128 &  13 25 23.71 & -43  3 26.75 & $ 0.06^{+ 0.51}_{- 0.06}$ & $ 1.64^{+1.21}_{-0.66}$ & $37.68^{+0.34}_{-0.09}$ & $  1.92$ & $   3$ \\
NGC5128 &  13 25 23.65 & -43  2 21.10 & $ 0.47^{+ 0.85}_{- 0.46}$ & $ 2.30^{+1.87}_{-1.21}$ & $37.80^{+1.07}_{-0.27}$ & $  0.85$ & $   2$ \\
NGC5128 &  13 25 23.60 & -43  1 39.09 & $ 0.00^{+ 0.74}_{- 0.00}$ & $ 1.20^{+1.32}_{-0.33}$ & $38.01^{+0.28}_{-0.09}$ & $  0.63$ & $   2$ \\
NGC5128 &  13 25 22.94 & -43  1 25.49 & $ 0.00^{+ 0.15}_{- 0.00}$ & $ 1.20^{+0.33}_{-0.22}$ & $38.17^{+0.06}_{-0.05}$ & $  4.93$ & $   5$ \\
NGC5128 &  13 25 18.58 & -43  1 16.97 & $ 0.27^{+ 1.25}_{- 0.27}$ & $ 1.86^{+1.76}_{-0.88}$ & $37.81^{+0.90}_{-0.14}$ & $  0.20$ & $   1$ \\
NGC5128 &  13 25 24.01 & -43  0 59.68 & $ 2.13^{+ 3.23}_{- 2.13}$ & $ 2.74^{+2.20}_{-1.76}$ & $38.59^{+1.92}_{-0.65}$ & $  1.28$ & $   3$ \\
NGC5194 &  13 30  7.56 & +47 11  5.68 & $ 0.07^{+ 0.03}_{- 0.05}$ & $ 1.97^{+0.11}_{-0.22}$ & $39.34^{+0.04}_{-0.03}$ & $ 49.09$ & $  36$ \\
NGC5194 &  13 30  6.50 & +47  8 34.60 & $ 0.11^{+ 0.14}_{- 0.11}$ & $ 2.08^{+0.44}_{-0.44}$ & $38.74^{+0.16}_{-0.09}$ & $  3.77$ & $   5$ \\
NGC5194 &  13 30  4.33 & +47 13 20.75 & $ 0.00^{+ 0.15}_{- 0.00}$ & $ 1.20^{+0.33}_{-0.33}$ & $38.57^{+0.08}_{-0.06}$ & $  1.39$ & $   2$ \\
NGC5194 &  13 29 57.56 & +47 10 48.32 & $ 0.11^{+ 0.13}_{- 0.11}$ & $ 1.75^{+0.55}_{-0.44}$ & $38.94^{+0.08}_{-0.04}$ & $ 10.26$ & $  10$ \\
NGC5194 &  13 29 56.26 & +47 14 51.49 & $ 0.00^{+ 0.35}_{- 0.00}$ & $ 1.31^{+1.21}_{-0.33}$ & $38.76^{+0.13}_{-0.11}$ & $  4.57$ & $   3$ \\
NGC5194 &  13 29 54.18 & +47 11 36.94 & $ 0.27^{+ 0.48}_{- 0.27}$ & $ 1.53^{+1.10}_{-0.77}$ & $38.43^{+0.31}_{-0.16}$ & $  3.92$ & $   3$ \\
NGC5194 &  13 29 53.79 & +47 14 31.45 & $ 0.03^{+ 0.88}_{- 0.03}$ & $ 2.19^{+4.84}_{-0.99}$ & $38.37^{+2.52}_{-0.08}$ & $  0.09$ & $   1$ \\
NGC5194 &  13 29 53.73 & +47 14 35.69 & $ 0.00^{+ 0.07}_{- 0.00}$ & $ 1.09^{+0.33}_{-0.11}$ & $39.14^{+0.04}_{-0.06}$ & $  5.99$ & $  15$ \\
NGC5194 &  13 29 53.31 & +47 10 42.38 & $ 0.00^{+ 0.04}_{- 0.00}$ & $ 1.42^{+0.11}_{-0.00}$ & $39.19^{+0.02}_{-0.03}$ & $ 19.26$ & $  24$ \\
NGC5194 &  13 29 51.36 & +47 10 32.28 & $ 0.08^{+ 0.21}_{- 0.08}$ & $ 1.20^{+0.66}_{-0.44}$ & $38.78^{+0.10}_{-0.10}$ & $  2.07$ & $   4$ \\
NGC5194 &  13 29 50.81 & +47 10 31.20 & $ 0.00^{+ 0.29}_{- 0.00}$ & $ 1.42^{+1.32}_{-0.66}$ & $38.27^{+0.26}_{-0.16}$ & $  1.49$ & $   2$ \\
NGC5194 &  13 29 50.66 & +47 11 54.95 & $ 3.92^{+ 1.44}_{- 1.27}$ & $ 1.97^{+0.66}_{-0.77}$ & $39.76^{+0.40}_{-0.23}$ & $  9.79$ & $   9$ \\
NGC5194 &  13 29 49.03 & +47 10 53.38 & $ 0.04^{+ 0.23}_{- 0.04}$ & $ 1.53^{+0.55}_{-0.33}$ & $38.58^{+0.12}_{-0.05}$ & $  1.77$ & $   3$ \\
NGC5194 &  13 29 43.35 & +47 15 25.33 & $ 0.02^{+ 0.33}_{- 0.02}$ & $ 1.97^{+1.87}_{-0.55}$ & $38.35^{+0.63}_{-0.06}$ & $  1.62$ & $   2$ \\
NGC5194 &  13 29 43.29 & +47 11 34.65 & $ 0.20^{+ 0.18}_{- 0.17}$ & $ 4.72^{+1.76}_{-1.76}$ & $39.52^{+0.85}_{-0.65}$ & $  9.81$ & $   9$ \\
NGC5194 &  13 29 39.45 & +47 12 43.60 & $ 0.01^{+ 0.13}_{- 0.01}$ & $ 1.53^{+0.44}_{-0.22}$ & $38.73^{+0.05}_{-0.08}$ & $ 13.28$ & $   6$ \\
NGC5194 &  13 29 38.63 & +47 13 36.16 & $ 0.18^{+ 0.56}_{- 0.18}$ & $ 3.51^{+3.30}_{-1.43}$ & $38.59^{+1.95}_{-0.42}$ & $  2.76$ & $   1$ \\
NGC5194 &  13 30 11.02 & +47 10 40.46 & $ 0.00^{+ 0.21}_{- 0.00}$ & $ 1.09^{+1.10}_{-0.66}$ & $38.39^{+0.30}_{-0.21}$ & $  1.32$ & $   2$ \\
NGC5457 &  14  3 36.10 & +54 19 23.92 & $ 0.00^{+ 0.47}_{- 0.00}$ & $ 2.19^{+3.52}_{-0.55}$ & $38.43^{+1.48}_{-0.06}$ & $  0.50$ & $   1$ \\
NGC5457 &  14  3 32.45 & +54 21  2.04 & $ 0.26^{+ 0.07}_{- 0.10}$ & $ 7.69^{+0.88}_{-1.21}$ & $40.40^{+0.40}_{-0.56}$ & $  3.65$ & $   8$ \\
NGC5457 &  14  3 24.25 & +54 19 48.02 & $ 0.42^{+ 0.90}_{- 0.42}$ & $ 1.20^{+1.32}_{-1.10}$ & $38.90^{+0.35}_{-0.13}$ & $  4.27$ & $   3$ \\
NGC5457 &  14  3 21.60 & +54 19 45.02 & $ 0.32^{+ 0.59}_{- 0.32}$ & $ 1.97^{+1.32}_{-0.88}$ & $38.89^{+0.58}_{-0.15}$ & $  0.46$ & $   1$ \\
NGC5775 &  14 54 13.24 & + 3 32 44.89 & $ 0.02^{+ 0.11}_{- 0.02}$ & $ 1.42^{+0.33}_{-0.22}$ & $39.49^{+0.05}_{-0.07}$ & $  9.67$ & $   6$ \\
NGC5775 &  14 54  0.97 & + 3 31 33.11 & $ 0.01^{+ 2.34}_{- 0.01}$ & $ 0.43^{+1.43}_{-0.44}$ & $39.68^{+0.23}_{-0.09}$ & $  2.35$ & $   2$ \\
NGC5775 &  14 54  0.96 & + 3 31 29.39 & $ 1.29^{+ 1.95}_{- 1.29}$ & $ 1.75^{+1.32}_{-0.99}$ & $39.64^{+0.76}_{-0.24}$ & $  0.62$ & $   3$ \\
NGC5775 &  14 53 59.45 & + 3 31 57.25 & $ 0.37^{+ 0.29}_{- 0.29}$ & $ 1.20^{+0.44}_{-0.44}$ & $39.85^{+0.05}_{-0.06}$ & $ 12.76$ & $  10$ \\
NGC5775 &  14 53 58.90 & + 3 32 16.78 & $ 2.75^{+ 0.34}_{- 0.30}$ & $ 1.86^{+0.22}_{-0.11}$ & $40.95^{+0.10}_{-0.06}$ & $ 60.08$ & $  57$ \\
NGC5775 &  14 53 56.80 & + 3 31 29.41 & $ 0.54^{+ 0.32}_{- 0.40}$ & $ 2.74^{+0.88}_{-0.88}$ & $39.54^{+0.51}_{-0.32}$ & $  5.56$ & $   3$ \\
NGC5775 &  14 53 55.92 & + 3 34  0.74 & $ 0.08^{+ 0.15}_{- 0.08}$ & $ 1.31^{+0.33}_{-0.22}$ & $39.71^{+0.05}_{-0.05}$ & $  7.01$ & $  11$ \\
NGC5775 &  14 53 55.76 & + 3 33 28.02 & $ 3.22^{+ 1.33}_{- 1.19}$ & $ 2.30^{+0.77}_{-0.77}$ & $40.36^{+0.53}_{-0.32}$ & $  7.77$ & $   7$ \\
NGC5775 &  14 53 55.25 & + 3 32 29.18 & $ 0.28^{+ 0.34}_{- 0.28}$ & $ 2.08^{+1.21}_{-1.10}$ & $39.44^{+0.45}_{-0.14}$ & $  0.43$ & $   3$ \\
NGC5775 &  14 53 54.75 & + 3 33 40.76 & $ 0.88^{+ 1.59}_{- 0.88}$ & $ 3.29^{+4.18}_{-2.75}$ & $39.59^{+3.07}_{-0.70}$ & $  0.59$ & $   1$ \\
NGC5775 &  14 53 53.71 & + 3 36 24.09 & $ 0.00^{+ 0.06}_{- 0.00}$ & $ 1.53^{+0.66}_{-0.44}$ & $39.16^{+0.09}_{-0.05}$ & $  3.64$ & $   1$ \\
NGC5775 &  14 53 53.14 & + 3 32 55.54 & $ 0.00^{+ 0.17}_{- 0.00}$ & $ 0.87^{+0.66}_{-0.55}$ & $39.32^{+0.13}_{-0.07}$ & $  6.23$ & $   3$ \\
NGC5775 &  14 53 48.29 & + 3 34  2.46 & $ 0.75^{+ 0.93}_{- 0.75}$ & $ 2.41^{+1.87}_{-1.65}$ & $39.56^{+1.15}_{-0.30}$ & $  2.10$ & $   1$ \\
NGC5775 &  14 53 44.70 & + 3 33 30.89 & $ 0.10^{+ 0.03}_{- 0.06}$ & $ 2.19^{+0.11}_{-0.22}$ & $40.01^{+0.03}_{-0.06}$ & $ 41.83$ & $  32$ \\
NGC5775 &  14 53 55.94 & + 3 29 12.83 & $ 0.05^{+ 0.40}_{- 0.05}$ & $ 1.64^{+1.32}_{-0.55}$ & $39.23^{+0.37}_{-0.07}$ & $  4.09$ & $   2$ \\
NGC6946 &  20 35  0.96 & +60 10 11.02 & $ 0.39^{+ 0.10}_{- 0.14}$ & $ 1.75^{+0.22}_{-0.33}$ & $38.55^{+0.05}_{-0.05}$ & $ 26.35$ & $  15$ \\
NGC6946 &  20 35  0.13 & +60  9  7.97 & $ 0.61^{+ 0.06}_{- 0.05}$ & $ 5.14^{+0.34}_{-0.27}$ & $40.41^{+0.21}_{-0.18}$ & $134.85$ & $  63$ \\
NGC6946 &  20 34 57.73 & +60  9 48.83 & $ 0.55^{+ 0.14}_{- 0.16}$ & $ 2.52^{+0.44}_{-0.44}$ & $38.69^{+0.19}_{-0.14}$ & $ 10.72$ & $  13$ \\
NGC6946 &  20 34 56.49 & +60  8 34.04 & $ 0.48^{+ 0.47}_{- 0.24}$ & $ 1.53^{+0.55}_{-0.33}$ & $38.62^{+0.17}_{-0.05}$ & $ 35.09$ & $  14$ \\
NGC6946 &  20 34 48.78 & +60  5 54.50 & $ 0.35^{+ 0.20}_{- 0.13}$ & $ 4.94^{+1.54}_{-0.77}$ & $39.27^{+0.89}_{-0.45}$ & $ 49.24$ & $  11$ \\
NGC6946 &  20 34 48.44 & +60  8 11.38 & $ 0.22^{+ 0.33}_{- 0.22}$ & $ 1.75^{+0.66}_{-0.55}$ & $38.22^{+0.18}_{-0.11}$ & $ 13.12$ & $   6$ \\
NGC6946 &  20 34 39.77 & +60  8 22.87 & $ 6.53^{+ 6.50}_{- 6.50}$ & $ 5.49^{+4.51}_{-4.07}$ & $40.91^{+4.10}_{-3.08}$ & $  0.84$ & $   1$ \\
NGC6946 &  20 34 36.48 & +60  9 30.46 & $ 0.50^{+ 0.06}_{- 0.05}$ & $ 4.61^{+0.33}_{-0.33}$ & $39.71^{+0.20}_{-0.19}$ & $ 59.19$ & $  31$ \\
NGC6946 &  20 34 34.42 & +60 10 33.08 & $ 0.31^{+ 0.30}_{- 0.31}$ & $ 3.51^{+1.43}_{-1.21}$ & $38.21^{+0.82}_{-0.55}$ & $  4.05$ & $   3$ \\
NGC6946 &  20 34 26.08 & +60  9  9.41 & $ 0.33^{+ 0.04}_{- 0.07}$ & $ 1.97^{+0.22}_{-0.11}$ & $38.85^{+0.04}_{-0.04}$ & $ 54.03$ & $  35$ \\
NGC6946 &  20 34 24.94 & +60  9  6.10 & $ 0.07^{+ 0.20}_{- 0.07}$ & $ 1.42^{+0.44}_{-0.33}$ & $38.10^{+0.06}_{-0.06}$ & $ 16.77$ & $   5$ \\
NGC6946 &  20 34 19.02 & +60 10  7.97 & $ 0.04^{+ 1.20}_{- 0.04}$ & $ 1.20^{+3.30}_{-0.99}$ & $37.69^{+1.32}_{-0.13}$ & $  0.29$ & $   1$ \\
NGC6946 &  20 35  5.32 & +60  6 23.10 & $ 0.16^{+ 0.84}_{- 0.16}$ & $ 1.42^{+0.99}_{-0.55}$ & $37.88^{+0.34}_{-0.09}$ & $  7.97$ & $   2$ \\
NGC6946 &  20 35  1.96 & +60 10  3.62 & $ 0.22^{+ 0.40}_{- 0.22}$ & $ 1.31^{+0.77}_{-0.55}$ & $38.14^{+0.12}_{-0.07}$ & $  2.07$ & $   4$ \\
NGC6946 &  20 34 24.71 & +60 10 38.83 & $ 0.94^{+ 4.99}_{- 0.94}$ & $ 0.65^{+2.20}_{-0.99}$ & $38.01^{+0.92}_{-0.09}$ & $  1.83$ & $   2$ \\
\enddata
\tablecomments{Host galaxy name; Right Ascension; Declination; $n_H$, equivalent hydrogen column density; $\Gamma$, photon power-law index; L, X-ray luminosity in the energy range: 0.3-8.0 keV; C-statistics; degree of freedom. }
\end{deluxetable}


==> tab5.tex <==
%\LongTables
\begin{deluxetable} {lccccccr}
\tablenum{5}
\tablewidth{0pc}
\tablecaption{Spectral Properties of point sources fitted with the disk black body model}
\tablehead{
\colhead{Galaxy} & \colhead{R.A.} & \colhead{Decl.} & \colhead{$n_H$($10^{22}cm^{-2}$)} & \colhead{kT$_{in}$ (keV)} & \colhead{log(L) ergs/s} & \colhead{C$_{stat}$} & \colhead{d. o. f.}}
\startdata
NGC0253 &  0 47 43.07 & -25 15 29.28 & $  0.00^{+ 0.32}_{-0.00}$ & $ 0.59^{+0.42}_{-0.25}$ & $37.69^{+0.37}_{-0.00}$ & $  9.41$ & $   4$ \\
NGC0253 &  0 47 42.80 & -25 15  2.02 & $  0.44^{+ 0.36}_{-0.32}$ & $ 1.56^{+1.95}_{-0.52}$ & $38.40^{+0.26}_{-0.08}$ & $  3.95$ & $   4$ \\
NGC0253 &  0 47 35.25 & -25 15 11.53 & $  0.24^{+ 0.07}_{-0.07}$ & $ 1.04^{+0.21}_{-0.15}$ & $38.71^{+0.04}_{-0.03}$ & $ 35.79$ & $  19$ \\
NGC0253 &  0 47 34.28 & -25 17  3.32 & $  3.08^{+ 5.36}_{-3.07}$ & $ 0.62^{+9.38}_{-0.36}$ & $38.69^{+2.04}_{-0.60}$ & $  3.37$ & $   2$ \\
NGC0253 &  0 47 34.00 & -25 16 36.51 & $  0.64^{+ 0.12}_{-0.10}$ & $ 1.34^{+0.19}_{-0.16}$ & $39.06^{+0.03}_{-0.03}$ & $  8.60$ & $  27$ \\
NGC0253 &  0 47 33.55 & -25 18 16.51 & $  0.00^{+ 0.08}_{-0.00}$ & $ 0.86^{+0.69}_{-0.29}$ & $37.49^{+0.20}_{-0.06}$ & $  3.85$ & $   2$ \\
NGC0253 &  0 47 32.05 & -25 17 21.43 & $  2.04^{+ 1.82}_{-1.62}$ & $ 2.07^{+4.71}_{-0.80}$ & $38.68^{+0.40}_{-0.09}$ & $  1.37$ & $   3$ \\
NGC0253 &  0 47 30.98 & -25 18 26.23 & $  0.96^{+ 0.96}_{-0.86}$ & $ 2.00^{+8.00}_{-0.91}$ & $38.41^{+0.73}_{-0.12}$ & $  1.84$ & $   3$ \\
NGC0253 &  0 47 28.01 & -25 18 20.21 & $  0.62^{+ 0.77}_{-0.56}$ & $ 1.20^{+8.80}_{-0.55}$ & $38.08^{+0.90}_{-0.12}$ & $  2.51$ & $   1$ \\
NGC0253 &  0 47 25.20 & -25 19 45.22 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.20^{+0.86}_{-0.33}$ & $38.12^{+0.21}_{-0.09}$ & $  7.71$ & $   4$ \\
NGC0253 &  0 47 18.50 & -25 19 13.94 & $  0.00^{+ 0.05}_{-0.00}$ & $ 1.59^{+0.73}_{-0.41}$ & $38.22^{+0.15}_{-0.09}$ & $  6.36$ & $   5$ \\
NGC0253 &  0 47 40.66 & -25 14 11.71 & $  0.42^{+ 0.47}_{-0.38}$ & $ 0.90^{+2.76}_{-0.40}$ & $37.94^{+0.38}_{-0.18}$ & $  1.64$ & $   3$ \\
NGC0253 &  0 47 17.65 & -25 18 26.45 & $  0.08^{+ 0.32}_{-0.07}$ & $ 1.24^{+8.76}_{-0.65}$ & $38.23^{+1.04}_{-0.13}$ & $  2.85$ & $   3$ \\
NGC0628 &  1 36 51.06 & +15 45 46.86 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.89^{+0.08}_{-0.11}$ & $39.42^{+0.02}_{-0.04}$ & $119.44$ & $  36$ \\
NGC0628 &  1 36 47.45 & +15 47 45.01 & $  0.75^{+ 0.58}_{-0.39}$ & $ 0.09^{+0.04}_{-0.03}$ & $41.65^{+2.49}_{-1.60}$ & $  0.66$ & $   4$ \\
NGC0628 &  1 36 44.12 & +15 48 18.85 & $  0.22^{+ 0.16}_{-0.16}$ & $ 0.99^{+0.29}_{-0.19}$ & $39.10^{+0.06}_{-0.06}$ & $  7.56$ & $   9$ \\
NGC0628 &  1 36 41.73 & +15 47  1.23 & $  0.00^{+ 0.14}_{-0.00}$ & $ 1.08^{+0.72}_{-0.37}$ & $38.31^{+0.19}_{-0.06}$ & $  4.70$ & $   3$ \\
NGC0628 &  1 36 41.66 & +15 45 52.30 & $  0.19^{+ 0.21}_{-0.17}$ & $ 1.01^{+0.78}_{-0.29}$ & $38.77^{+0.11}_{-0.07}$ & $ 14.10$ & $   3$ \\
NGC0628 &  1 36 39.10 & +15 43  9.86 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.25^{+0.30}_{-0.22}$ & $38.89^{+0.07}_{-0.04}$ & $  5.67$ & $   6$ \\
NGC0628 &  1 36 25.13 & +15 48 59.87 & $  0.48^{+ 0.91}_{-0.45}$ & $ 0.60^{+0.71}_{-0.24}$ & $38.87^{+0.61}_{-0.21}$ & $  0.31$ & $   1$ \\
NGC0891 &  2 22 37.08 & +42 21 58.24 & $  0.26^{+ 0.19}_{-0.18}$ & $ 1.15^{+0.52}_{-0.27}$ & $39.02^{+0.06}_{-0.09}$ & $  3.52$ & $   7$ \\
NGC0891 &  2 22 35.74 & +42 20 52.91 & $  0.52^{+ 0.39}_{-0.36}$ & $ 0.91^{+0.62}_{-0.26}$ & $38.85^{+0.17}_{-0.13}$ & $  0.37$ & $   2$ \\
NGC0891 &  2 22 34.40 & +42 21  0.39 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.11^{+0.30}_{-0.22}$ & $38.81^{+0.08}_{-0.04}$ & $  4.88$ & $   5$ \\
NGC0891 &  2 22 31.91 & +42 22 34.68 & $  0.00^{+ 0.01}_{-0.00}$ & $ 2.44^{+6.09}_{-1.19}$ & $38.56^{+0.65}_{-0.25}$ & $  4.13$ & $   2$ \\
NGC0891 &  2 22 31.35 & +42 20 24.33 & $  0.43^{+ 0.04}_{-0.04}$ & $ 1.58^{+0.14}_{-0.10}$ & $40.15^{+0.02}_{-0.02}$ & $105.31$ & $  83$ \\
NGC0891 &  2 22 31.26 & +42 19 57.79 & $  0.23^{+ 0.05}_{-0.04}$ & $ 1.30^{+0.09}_{-0.11}$ & $39.91^{+0.02}_{-0.02}$ & $139.40$ & $  62$ \\
NGC0891 &  2 22 28.98 & +42 20 22.22 & $  0.00^{+ 0.02}_{-0.00}$ & $ 2.36^{+7.64}_{-0.96}$ & $38.87^{+0.75}_{-0.20}$ & $  3.65$ & $   2$ \\
NGC0891 &  2 22 27.58 & +42 21  8.84 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.01^{+0.23}_{-0.17}$ & $38.72^{+0.05}_{-0.03}$ & $ 12.62$ & $   6$ \\
NGC0891 &  2 22 26.28 & +42 18 33.69 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.89^{+0.51}_{-0.24}$ & $38.38^{+0.16}_{-0.02}$ & $  8.10$ & $   4$ \\
NGC0891 &  2 22 25.26 & +42 24 51.64 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.14^{+0.08}_{-0.10}$ & $39.55^{+0.02}_{-0.02}$ & $ 56.09$ & $  43$ \\
NGC0891 &  2 22 24.36 & +42 21 38.98 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.94^{+0.11}_{-0.08}$ & $39.24^{+0.03}_{-0.02}$ & $ 28.27$ & $  24$ \\
NGC0891 &  2 22 15.11 & +42 20 45.01 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.91^{+0.16}_{-0.15}$ & $39.05^{+0.04}_{-0.04}$ & $ 42.63$ & $  16$ \\
NGC0891 &  2 22 15.04 & +42 23 41.75 & $  0.00^{+ 0.02}_{-0.00}$ & $ 0.97^{+0.31}_{-0.22}$ & $38.60^{+0.07}_{-0.04}$ & $  5.83$ & $   3$ \\
NGC0891 &  2 22 42.13 & +42 24  3.02 & $  0.05^{+ 0.09}_{-0.05}$ & $ 2.18^{+7.82}_{-0.98}$ & $39.04^{+0.80}_{-0.21}$ & $  0.82$ & $   5$ \\
NGC1291 &  3 17 26.34 & -41  5 44.53 & $  0.00^{+ 0.03}_{-0.00}$ & $ 0.80^{+0.39}_{-0.19}$ & $38.26^{+0.13}_{-0.05}$ & $ 10.52$ & $   4$ \\
NGC1291 &  3 17 23.45 & -41  6 49.13 & $  0.00^{+ 0.23}_{-0.00}$ & $ 1.13^{+8.87}_{-0.70}$ & $38.36^{+1.16}_{-0.17}$ & $  1.35$ & $   1$ \\
NGC1291 &  3 17 21.69 & -41  6 52.34 & $  0.00^{+ 0.13}_{-0.00}$ & $ 1.65^{+1.98}_{-0.65}$ & $38.66^{+0.37}_{-0.16}$ & $  3.07$ & $   2$ \\
NGC1291 &  3 17 21.43 & -41  7 34.42 & $  0.00^{+ 0.07}_{-0.00}$ & $ 1.91^{+2.54}_{-0.65}$ & $38.58^{+0.38}_{-0.15}$ & $  4.59$ & $   4$ \\
NGC1291 &  3 17 19.35 & -41  6 14.92 & $  0.00^{+ 0.08}_{-0.00}$ & $ 1.53^{+0.95}_{-0.42}$ & $38.67^{+0.20}_{-0.10}$ & $  7.38$ & $   3$ \\
NGC1291 &  3 17 17.50 & -41  7 18.72 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.36^{+0.14}_{-0.09}$ & $38.08^{+0.18}_{-0.01}$ & $  3.77$ & $   1$ \\
NGC1291 &  3 17 16.66 & -41  5 13.36 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.35^{+0.06}_{-0.06}$ & $38.42^{+0.16}_{-0.01}$ & $  9.28$ & $   3$ \\
NGC1291 &  3 17 16.51 & -41  7 13.22 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.30^{+1.25}_{-0.43}$ & $38.24^{+0.27}_{-0.14}$ & $  3.14$ & $   2$ \\
NGC1291 &  3 17 14.98 & -41  6 12.37 & $  0.00^{+ 0.08}_{-0.00}$ & $ 2.45^{+7.55}_{-1.24}$ & $38.94^{+0.77}_{-0.30}$ & $  4.49$ & $   3$ \\
NGC1291 &  3 17 13.81 & -41  7 26.55 & $  0.00^{+ 0.12}_{-0.00}$ & $ 1.22^{+1.82}_{-0.49}$ & $38.56^{+0.43}_{-0.11}$ & $  1.10$ & $   2$ \\
NGC1291 &  3 17  8.85 & -41  5 34.19 & $  0.43^{+ 1.16}_{-0.43}$ & $ 0.70^{+9.30}_{-0.39}$ & $38.43^{+1.02}_{-0.21}$ & $  0.57$ & $   1$ \\
NGC1291 &  3 17  2.53 & -41  7 13.98 & $  0.01^{+ 0.04}_{-0.01}$ & $ 0.65^{+0.10}_{-0.10}$ & $39.14^{+0.04}_{-0.02}$ & $ 26.29$ & $  23$ \\
NGC1291 &  3 17 23.83 & -41  9 50.75 & $  0.00^{+ 0.08}_{-0.00}$ & $ 0.76^{+9.24}_{-0.07}$ & $38.19^{+1.31}_{-0.02}$ & $  2.90$ & $   2$ \\
NGC1291 &  3 17 22.36 & -41  9 25.62 & $  0.01^{+ 0.19}_{-0.01}$ & $10.00^{+0.00}_{-7.94}$ & $39.50^{+0.08}_{-0.78}$ & $  5.37$ & $   2$ \\
NGC1316 &  3 22 51.23 & -37  9 49.43 & $  0.08^{+ 0.07}_{-0.07}$ & $ 0.34^{+0.10}_{-0.05}$ & $39.61^{+0.17}_{-0.15}$ & $  7.41$ & $   9$ \\
NGC1316 &  3 22 42.68 & -37 12 17.11 & $  0.25^{+ 0.45}_{-0.23}$ & $ 0.37^{+0.41}_{-0.15}$ & $39.14^{+0.79}_{-0.28}$ & $  1.72$ & $   2$ \\
NGC1316 &  3 22 42.46 & -37 12 21.56 & $  0.00^{+ 0.08}_{-0.00}$ & $ 0.54^{+0.30}_{-0.14}$ & $38.98^{+0.11}_{-0.00}$ & $  4.36$ & $   2$ \\
NGC1316 &  3 22 42.09 & -37 11 23.18 & $  0.00^{+ 0.19}_{-0.00}$ & $ 1.31^{+1.01}_{-0.47}$ & $39.06^{+0.21}_{-0.11}$ & $  1.11$ & $   1$ \\
NGC1316 &  3 22 40.77 & -37 12 23.94 & $  0.00^{+ 0.03}_{-0.00}$ & $ 1.16^{+0.56}_{-0.50}$ & $39.13^{+0.16}_{-0.09}$ & $ 17.41$ & $   3$ \\
NGC1316 &  3 22 40.50 & -37 12 26.71 & $  0.00^{+ 0.25}_{-0.00}$ & $ 0.31^{+0.09}_{-0.14}$ & $38.85^{+0.82}_{-0.03}$ & $  3.62$ & $   3$ \\
NGC1316 &  3 22 36.43 & -37 13 23.75 & $  0.00^{+ 0.09}_{-0.00}$ & $ 0.56^{+0.56}_{-0.18}$ & $38.91^{+0.18}_{-0.01}$ & $  3.77$ & $   1$ \\
NGC1316 &  3 22 35.55 & -37 13 13.17 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.47^{+0.18}_{-0.10}$ & $38.95^{+0.10}_{-0.00}$ & $  7.13$ & $   2$ \\
NGC1316 &  3 22 25.70 & -37  9 12.36 & $  0.00^{+ 0.02}_{-0.00}$ & $ 0.42^{+0.08}_{-0.08}$ & $39.23^{+0.05}_{-0.00}$ & $  7.97$ & $   4$ \\
NGC1399 &  3 38 51.61 & -35 26 43.59 & $  0.00^{+ 0.00}_{-0.00}$ & $ 1.17^{+0.11}_{-0.10}$ & $40.04^{+0.03}_{-0.02}$ & $ 80.79$ & $  48$ \\
NGC1399 &  3 38 48.71 & -35 28 34.34 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.45^{+0.06}_{-0.06}$ & $39.16^{+0.02}_{-0.01}$ & $ 24.67$ & $   9$ \\
NGC1399 &  3 38 45.35 & -35 27 37.07 & $  0.07^{+ 0.11}_{-0.06}$ & $ 1.14^{+0.50}_{-0.29}$ & $39.17^{+0.10}_{-0.08}$ & $  5.66$ & $   4$ \\
NGC1399 &  3 38 44.96 & -35 28 21.50 & $  0.00^{+ 0.11}_{-0.00}$ & $ 0.90^{+1.50}_{-0.36}$ & $38.59^{+0.42}_{-0.08}$ & $  1.44$ & $   2$ \\
NGC1399 &  3 38 41.37 & -35 31 34.06 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.98^{+0.04}_{-0.06}$ & $40.48^{+0.01}_{-0.01}$ & $404.64$ & $  98$ \\
NGC1399 &  3 38 38.80 & -35 25 54.39 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.88^{+0.56}_{-0.25}$ & $38.73^{+0.18}_{-0.06}$ & $  1.52$ & $   2$ \\
NGC1399 &  3 38 38.62 & -35 27 27.58 & $  0.08^{+ 0.30}_{-0.07}$ & $ 0.74^{+2.26}_{-0.34}$ & $38.58^{+0.49}_{-0.09}$ & $  2.80$ & $   2$ \\
NGC1399 &  3 38 36.83 & -35 27 46.75 & $  0.00^{+ 0.03}_{-0.00}$ & $ 0.39^{+0.07}_{-0.06}$ & $38.93^{+0.08}_{-0.00}$ & $ 14.37$ & $   4$ \\
NGC1399 &  3 38 36.34 & -35 27  8.40 & $  0.00^{+ 0.07}_{-0.00}$ & $ 0.69^{+0.32}_{-0.19}$ & $38.62^{+0.08}_{-0.02}$ & $  4.62$ & $   3$ \\
NGC1399 &  3 38 36.30 & -35 28  9.19 & $  0.00^{+ 0.32}_{-0.00}$ & $ 2.87^{+7.13}_{-1.38}$ & $39.15^{+0.66}_{-0.25}$ & $  3.72$ & $   2$ \\
NGC1399 &  3 38 36.17 & -35 26 25.11 & $  0.00^{+ 0.15}_{-0.00}$ & $ 0.56^{+0.75}_{-0.31}$ & $38.40^{+0.33}_{-0.17}$ & $  1.86$ & $   2$ \\
NGC1399 &  3 38 33.82 & -35 25 56.43 & $  0.00^{+ 0.09}_{-0.00}$ & $ 0.58^{+0.24}_{-0.17}$ & $38.67^{+0.13}_{-0.03}$ & $  2.59$ & $   2$ \\
NGC1399 &  3 38 33.80 & -35 26 57.96 & $  0.01^{+ 0.16}_{-0.01}$ & $ 0.79^{+0.43}_{-0.29}$ & $38.60^{+0.17}_{-0.05}$ & $  1.72$ & $   3$ \\
NGC1399 &  3 38 33.18 & -35 25 53.26 & $  0.00^{+ 0.11}_{-0.00}$ & $ 0.94^{+9.06}_{-0.18}$ & $38.57^{+1.16}_{-0.09}$ & $  2.47$ & $   2$ \\
NGC1399 &  3 38 33.12 & -35 27 31.29 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.85^{+0.17}_{-0.13}$ & $39.14^{+0.07}_{-0.04}$ & $ 23.22$ & $   7$ \\
NGC1399 &  3 38 32.80 & -35 26 58.29 & $  0.01^{+ 0.15}_{-0.01}$ & $ 1.19^{+2.19}_{-0.56}$ & $38.98^{+0.45}_{-0.20}$ & $  0.05$ & $   2$ \\
NGC1399 &  3 38 32.60 & -35 27  5.12 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.28^{+0.18}_{-0.13}$ & $39.76^{+0.05}_{-0.03}$ & $ 29.26$ & $  26$ \\
NGC1399 &  3 38 32.35 & -35 27  1.75 & $  0.28^{+ 0.34}_{-0.22}$ & $ 0.70^{+0.70}_{-0.25}$ & $38.91^{+0.24}_{-0.16}$ & $  4.42$ & $   2$ \\
NGC1399 &  3 38 32.33 & -35 26 45.73 & $  0.01^{+ 0.13}_{-0.01}$ & $ 0.18^{+0.05}_{-0.06}$ & $38.70^{+0.73}_{-0.09}$ & $ 10.61$ & $   1$ \\
NGC1399 &  3 38 32.34 & -35 27 10.34 & $  0.07^{+ 0.28}_{-0.06}$ & $ 0.99^{+1.77}_{-0.45}$ & $38.90^{+0.35}_{-0.14}$ & $  0.24$ & $   1$ \\
NGC1399 &  3 38 31.90 & -35 26 49.04 & $  0.00^{+ 0.03}_{-0.00}$ & $ 0.30^{+0.06}_{-0.08}$ & $38.90^{+0.10}_{-0.01}$ & $ 26.29$ & $   3$ \\
NGC1399 &  3 38 31.82 & -35 26  3.76 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.38^{+0.03}_{-0.02}$ & $39.44^{+0.04}_{-0.00}$ & $ 34.78$ & $  19$ \\
NGC1399 &  3 38 31.73 & -35 30 58.65 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.25^{+0.06}_{-0.06}$ & $38.82^{+0.26}_{-0.02}$ & $  4.66$ & $   2$ \\
NGC1399 &  3 38 29.84 & -35 27 48.02 & $  0.00^{+ 0.07}_{-0.00}$ & $ 1.89^{+4.53}_{-0.70}$ & $38.85^{+0.57}_{-0.16}$ & $  3.93$ & $   3$ \\
NGC1399 &  3 38 29.68 & -35 25  4.10 & $  0.00^{+ 0.05}_{-0.00}$ & $ 0.78^{+0.36}_{-0.23}$ & $39.04^{+0.11}_{-0.06}$ & $ 11.05$ & $   5$ \\
NGC1399 &  3 38 27.76 & -35 27 50.20 & $  0.00^{+ 0.19}_{-0.00}$ & $10.00^{+0.00}_{-8.66}$ & $39.94^{+0.05}_{-0.98}$ & $  4.41$ & $   2$ \\
NGC1399 &  3 38 27.64 & -35 26 48.16 & $  0.02^{+ 0.03}_{-0.02}$ & $ 0.42^{+0.07}_{-0.06}$ & $39.42^{+0.07}_{-0.04}$ & $ 38.17$ & $  19$ \\
NGC1399 &  3 38 27.17 & -35 26  0.91 & $  0.00^{+ 0.19}_{-0.00}$ & $ 0.82^{+1.70}_{-0.39}$ & $38.70^{+0.50}_{-0.06}$ & $  7.46$ & $   1$ \\
NGC1399 &  3 38 26.50 & -35 27 31.91 & $  0.02^{+ 0.20}_{-0.02}$ & $ 0.69^{+0.50}_{-0.28}$ & $38.92^{+0.22}_{-0.04}$ & $  0.37$ & $   2$ \\
NGC1399 &  3 38 25.94 & -35 27 41.77 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.84^{+0.51}_{-0.26}$ & $38.77^{+0.17}_{-0.04}$ & $  4.31$ & $   2$ \\
NGC1399 &  3 38 25.28 & -35 27 52.97 & $  0.00^{+ 0.12}_{-0.00}$ & $ 1.42^{+1.21}_{-0.47}$ & $38.81^{+0.23}_{-0.15}$ & $  3.64$ & $   4$ \\
NGC1399 &  3 38 25.29 & -35 25 21.92 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.48^{+0.12}_{-0.07}$ & $39.09^{+0.03}_{-0.01}$ & $ 40.19$ & $   9$ \\
NGC1399 &  3 38 21.91 & -35 29 28.30 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.29^{+0.59}_{-0.34}$ & $39.19^{+0.16}_{-0.10}$ & $ 14.79$ & $   5$ \\
NGC1399 &  3 38 31.68 & -35 26  0.22 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.77^{+0.39}_{-0.19}$ & $38.63^{+0.15}_{-0.03}$ & $  2.18$ & $   4$ \\
NGC1399 &  3 38 28.96 & -35 26  2.00 & $  0.00^{+ 0.07}_{-0.00}$ & $ 1.48^{+1.44}_{-0.46}$ & $38.89^{+0.28}_{-0.14}$ & $  1.55$ & $   4$ \\
NGC1399 &  3 38 25.62 & -35 25 55.34 & $  0.25^{+ 0.56}_{-0.24}$ & $ 0.52^{+1.08}_{-0.24}$ & $38.71^{+0.66}_{-0.21}$ & $  0.03$ & $   1$ \\
NGC1569 &  4 31 25.17 & +64 51 54.10 & $  5.61^{+ 1.08}_{-1.23}$ & $ 2.93^{+7.07}_{-0.97}$ & $38.54^{+0.52}_{-0.09}$ & $  5.01$ & $  15$ \\
NGC1569 &  4 31 20.52 & +64 51 22.51 & $  0.12^{+ 0.17}_{-0.11}$ & $ 1.56^{+1.65}_{-0.51}$ & $37.40^{+0.26}_{-0.09}$ & $  1.54$ & $   6$ \\
NGC1569 &  4 31 14.56 & +64 50 24.52 & $  0.27^{+ 1.10}_{-0.24}$ & $ 1.46^{+1.60}_{-0.60}$ & $37.06^{+0.19}_{-0.11}$ & $  1.75$ & $   3$ \\
NGC1569 &  4 31 14.02 & +64 51  7.94 & $  0.14^{+ 0.05}_{-0.04}$ & $ 0.22^{+0.02}_{-0.03}$ & $38.05^{+0.18}_{-0.12}$ & $ 74.53$ & $  29$ \\
NGC1569 &  4 31 13.21 & +64 52 29.54 & $  0.05^{+ 0.06}_{-0.05}$ & $ 1.14^{+0.22}_{-0.17}$ & $37.59^{+0.04}_{-0.07}$ & $ 13.01$ & $  17$ \\
NGC1569 &  4 30 58.37 & +64 48 52.37 & $  0.51^{+ 0.42}_{-0.40}$ & $ 0.21^{+0.19}_{-0.07}$ & $37.49^{+1.12}_{-0.81}$ & $  5.00$ & $   2$ \\
NGC1569 &  4 30 57.42 & +64 50 48.62 & $  0.46^{+ 0.24}_{-0.24}$ & $ 1.01^{+0.35}_{-0.19}$ & $37.57^{+0.08}_{-0.08}$ & $  5.94$ & $   9$ \\
NGC1569 &  4 30 49.86 & +64 50 55.48 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.97^{+0.99}_{-0.48}$ & $37.43^{+0.18}_{-0.10}$ & $ 10.22$ & $   7$ \\
NGC1569 &  4 30 48.62 & +64 50 58.59 & $  0.10^{+ 0.04}_{-0.05}$ & $ 1.68^{+0.30}_{-0.19}$ & $37.96^{+0.04}_{-0.04}$ & $ 50.02$ & $  33$ \\
NGC1569 &  4 30 48.26 & +64 50 46.65 & $  0.23^{+ 0.22}_{-0.20}$ & $ 2.00^{+3.34}_{-0.65}$ & $37.56^{+0.41}_{-0.11}$ & $ 17.20$ & $   7$ \\
NGC1569 &  4 30 48.14 & +64 50 50.57 & $  0.19^{+ 0.02}_{-0.03}$ & $ 0.41^{+0.04}_{-0.03}$ & $38.13^{+0.04}_{-0.05}$ & $ 97.93$ & $  50$ \\
NGC1569 &  4 30 34.33 & +64 47 40.56 & $  0.18^{+ 0.08}_{-0.08}$ & $ 1.21^{+0.26}_{-0.17}$ & $37.71^{+0.04}_{-0.06}$ & $ 20.43$ & $  18$ \\
NGC1569 &  4 30 30.88 & +64 52  5.38 & $  0.00^{+ 0.08}_{-0.00}$ & $ 1.89^{+0.70}_{-0.45}$ & $37.43^{+0.13}_{-0.12}$ & $  7.99$ & $   7$ \\
NGC1569 &  4 30 25.27 & +64 50 35.72 & $  0.58^{+ 1.30}_{-0.52}$ & $ 0.77^{+1.46}_{-0.34}$ & $37.12^{+0.59}_{-0.17}$ & $  1.38$ & $   1$ \\
NGC1569 &  4 31 24.43 & +64 51 15.89 & $  0.29^{+ 0.48}_{-0.26}$ & $ 1.18^{+1.34}_{-0.42}$ & $36.92^{+0.14}_{-0.13}$ & $  1.28$ & $   3$ \\
NGC2403 &  7 37 14.94 & +65 34 28.83 & $  0.19^{+ 0.58}_{-0.17}$ & $ 1.25^{+8.75}_{-0.70}$ & $37.70^{+1.02}_{-0.18}$ & $  1.37$ & $   1$ \\
NGC2403 &  7 37 11.63 & +65 33 45.52 & $  0.28^{+ 0.16}_{-0.14}$ & $ 1.09^{+0.23}_{-0.15}$ & $38.40^{+0.05}_{-0.05}$ & $ 19.06$ & $  13$ \\
NGC2403 &  7 36 42.03 & +65 36 51.99 & $  0.71^{+ 0.26}_{-0.28}$ & $ 0.10^{+0.03}_{-0.02}$ & $40.50^{+1.09}_{-1.05}$ & $ 11.36$ & $   7$ \\
NGC2403 &  7 36 32.91 & +65 34 58.01 & $  0.12^{+ 0.39}_{-0.12}$ & $ 0.42^{+3.48}_{-0.22}$ & $37.44^{+0.85}_{-0.16}$ & $  2.25$ & $   2$ \\
NGC3034 &  9 56 19.57 & +69 41 45.50 & $  0.40^{+ 0.45}_{-0.36}$ & $ 1.32^{+1.47}_{-0.42}$ & $38.38^{+0.17}_{-0.08}$ & $  0.43$ & $   3$ \\
NGC3034 &  9 55 54.55 & +69 41  0.39 & $  2.81^{+ 0.98}_{-0.90}$ & $ 1.41^{+0.62}_{-0.30}$ & $39.22^{+0.11}_{-0.06}$ & $  8.06$ & $  13$ \\
NGC3034 &  9 55 37.94 & +69 40 28.87 & $  0.08^{+ 0.48}_{-0.07}$ & $ 1.22^{+0.71}_{-0.41}$ & $38.12^{+0.15}_{-0.06}$ & $  0.51$ & $   2$ \\
NGC3034 &  9 55 27.00 & +69 39 23.15 & $  0.06^{+ 0.23}_{-0.06}$ & $ 1.25^{+0.42}_{-0.29}$ & $38.44^{+0.06}_{-0.05}$ & $  5.10$ & $   7$ \\
NGC3034 &  9 55 20.70 & +69 44 42.97 & $  0.46^{+ 1.09}_{-0.46}$ & $ 0.42^{+0.52}_{-0.20}$ & $38.32^{+1.18}_{-0.32}$ & $  0.15$ & $   3$ \\
NGC3079 & 10  2  5.39 & +55 42 58.29 & $  0.23^{+ 0.53}_{-0.20}$ & $ 2.85^{+7.15}_{-1.17}$ & $39.96^{+0.60}_{-0.17}$ & $  2.45$ & $   4$ \\
NGC3079 & 10  2  2.88 & +55 38 58.82 & $  0.00^{+ 0.04}_{-0.00}$ & $ 1.85^{+0.87}_{-0.46}$ & $39.86^{+0.18}_{-0.13}$ & $  7.54$ & $  12$ \\
NGC3079 & 10  1 58.11 & +55 41  3.65 & $  0.00^{+ 0.19}_{-0.00}$ & $ 0.79^{+0.59}_{-0.27}$ & $38.96^{+0.15}_{-0.02}$ & $  1.65$ & $   3$ \\
NGC3079 & 10  1 52.11 & +55 39  5.24 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.89^{+0.45}_{-0.22}$ & $39.00^{+0.12}_{-0.04}$ & $  4.71$ & $   2$ \\
NGC3079 & 10  2  1.01 & +55 36 48.20 & $  0.00^{+ 0.04}_{-0.00}$ & $ 0.69^{+0.23}_{-0.13}$ & $39.27^{+0.05}_{-0.02}$ & $ 11.45$ & $   3$ \\
NGC3379 & 10 47 52.78 & +12 35  8.46 & $  0.00^{+ 0.04}_{-0.00}$ & $ 0.87^{+0.38}_{-0.20}$ & $38.59^{+0.09}_{-0.04}$ & $  6.57$ & $   2$ \\
NGC3379 & 10 47 52.66 & +12 33 37.77 & $  0.02^{+ 0.12}_{-0.02}$ & $ 0.83^{+0.48}_{-0.28}$ & $38.98^{+0.12}_{-0.06}$ & $  3.38$ & $   4$ \\
NGC3379 & 10 47 49.11 & +12 34 48.72 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.06^{+0.39}_{-0.23}$ & $39.01^{+0.10}_{-0.05}$ & $  7.35$ & $   5$ \\
NGC3379 & 10 47 47.98 & +12 34 45.69 & $  0.57^{+ 0.74}_{-0.41}$ & $ 0.16^{+0.12}_{-0.06}$ & $39.85^{+2.13}_{-1.11}$ & $  1.53$ & $   2$ \\
NGC3379 & 10 47 46.96 & +12 34 38.61 & $  0.00^{+ 0.02}_{-0.00}$ & $ 0.47^{+0.09}_{-0.06}$ & $38.84^{+0.04}_{-0.00}$ & $  6.80$ & $   5$ \\
NGC3379 & 10 47 46.82 & +12 34 27.23 & $  0.27^{+ 0.46}_{-0.24}$ & $ 0.67^{+1.01}_{-0.29}$ & $38.72^{+0.39}_{-0.17}$ & $  0.31$ & $   1$ \\
NGC3379 & 10 47 41.85 & +12 37 45.36 & $  0.43^{+ 0.27}_{-0.23}$ & $ 0.14^{+0.06}_{-0.04}$ & $40.30^{+1.07}_{-0.82}$ & $  9.21$ & $   4$ \\
NGC3556 & 11 11 48.99 & +55 40 24.45 & $  0.06^{+ 0.34}_{-0.05}$ & $ 0.76^{+2.52}_{-0.39}$ & $38.46^{+0.56}_{-0.08}$ & $  0.81$ & $   2$ \\
NGC3556 & 11 11 41.41 & +55 40 57.74 & $  0.43^{+ 0.65}_{-0.39}$ & $ 1.52^{+2.01}_{-0.55}$ & $39.50^{+0.25}_{-0.07}$ & $  4.73$ & $   7$ \\
NGC3556 & 11 11 40.50 & +55 40 12.83 & $  0.07^{+ 0.40}_{-0.06}$ & $ 0.76^{+0.43}_{-0.28}$ & $38.84^{+0.27}_{-0.05}$ & $  1.85$ & $   2$ \\
NGC3556 & 11 11 39.02 & +55 41  2.58 & $  0.66^{+ 0.55}_{-0.65}$ & $ 0.12^{+0.09}_{-0.04}$ & $40.87^{+1.64}_{-2.27}$ & $ 16.69$ & $   3$ \\
NGC3556 & 11 11 38.39 & +55 39 51.79 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.48^{+0.72}_{-0.38}$ & $38.88^{+0.14}_{-0.08}$ & $  5.61$ & $   2$ \\
NGC3556 & 11 11 38.21 & +55 42 36.84 & $  0.80^{+ 0.45}_{-0.51}$ & $ 2.37^{+3.42}_{-0.74}$ & $39.66^{+0.33}_{-0.09}$ & $  9.79$ & $   8$ \\
NGC3556 & 11 11 38.15 & +55 40 19.23 & $  0.00^{+ 0.19}_{-0.00}$ & $ 0.74^{+0.31}_{-0.25}$ & $38.91^{+0.14}_{-0.02}$ & $  2.97$ & $   4$ \\
NGC3556 & 11 11 35.26 & +55 41  7.28 & $  0.02^{+ 0.41}_{-0.02}$ & $ 1.63^{+8.37}_{-1.07}$ & $38.91^{+1.00}_{-0.26}$ & $  0.52$ & $   2$ \\
NGC3556 & 11 11 30.34 & +55 40 31.29 & $  0.08^{+ 0.11}_{-0.08}$ & $ 1.56^{+0.47}_{-0.27}$ & $39.51^{+0.06}_{-0.07}$ & $ 12.85$ & $  12$ \\
NGC3556 & 11 11 26.90 & +55 39 14.83 & $  0.00^{+ 0.02}_{-0.00}$ & $ 1.00^{+0.19}_{-0.14}$ & $39.09^{+0.04}_{-0.03}$ & $ 10.95$ & $   8$ \\
NGC3556 & 11 11 26.82 & +55 40 28.78 & $  0.00^{+ 0.20}_{-0.00}$ & $ 0.97^{+0.44}_{-0.30}$ & $38.73^{+0.13}_{-0.05}$ & $  0.93$ & $   3$ \\
NGC3556 & 11 11 26.05 & +55 40 16.79 & $  0.16^{+ 0.04}_{-0.03}$ & $ 1.28^{+0.10}_{-0.12}$ & $40.00^{+0.02}_{-0.02}$ & $ 48.83$ & $  54$ \\
NGC3556 & 11 11 17.71 & +55 40  9.83 & $  0.00^{+ 0.04}_{-0.00}$ & $ 0.87^{+0.16}_{-0.15}$ & $39.09^{+0.04}_{-0.04}$ & $  5.55$ & $   9$ \\
NGC3556 & 11 11 25.74 & +55 44  1.58 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.77^{+0.10}_{-0.12}$ & $39.27^{+0.02}_{-0.03}$ & $ 46.12$ & $  15$ \\
NGC3556 & 11 11 17.87 & +55 40 17.08 & $  0.00^{+ 0.51}_{-0.00}$ & $ 8.83^{+1.17}_{-7.12}$ & $39.90^{+0.15}_{-0.69}$ & $  1.72$ & $   3$ \\
NGC3628 & 11 20 26.72 & +13 34 58.22 & $  0.00^{+ 0.14}_{-0.00}$ & $ 1.72^{+2.08}_{-0.59}$ & $38.35^{+0.34}_{-0.14}$ & $  5.08$ & $   2$ \\
NGC3628 & 11 20 24.38 & +13 38 22.94 & $  0.00^{+ 0.15}_{-0.00}$ & $ 1.31^{+0.33}_{-0.24}$ & $38.92^{+0.08}_{-0.03}$ & $  4.39$ & $   6$ \\
NGC3628 & 11 20 20.72 & +13 35  7.57 & $  1.78^{+ 2.06}_{-1.69}$ & $ 1.28^{+3.25}_{-0.54}$ & $39.10^{+0.35}_{-0.16}$ & $  2.15$ & $   3$ \\
NGC3628 & 11 20 16.25 & +13 35 27.20 & $  0.63^{+ 0.50}_{-0.55}$ & $ 1.76^{+2.65}_{-0.58}$ & $39.18^{+0.29}_{-0.08}$ & $  0.24$ & $   6$ \\
NGC3628 & 11 20 15.80 & +13 37 47.67 & $  0.00^{+ 0.03}_{-0.00}$ & $ 1.07^{+0.34}_{-0.21}$ & $38.73^{+0.06}_{-0.05}$ & $ 23.33$ & $   4$ \\
NGC3628 & 11 20 14.72 & +13 32 27.71 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.70^{+0.09}_{-0.06}$ & $39.13^{+0.03}_{-0.01}$ & $ 94.95$ & $  27$ \\
NGC3628 & 11 20 13.61 & +13 34 40.95 & $  0.49^{+ 0.50}_{-0.43}$ & $ 1.81^{+8.19}_{-0.83}$ & $39.06^{+0.80}_{-0.15}$ & $  5.38$ & $   4$ \\
NGC3628 & 11 20 13.35 & +13 35  8.52 & $  0.34^{+ 0.57}_{-0.30}$ & $ 3.27^{+6.73}_{-1.79}$ & $38.77^{+0.63}_{-0.20}$ & $  2.27$ & $   3$ \\
NGC3628 & 11 20 11.21 & +13 34 45.79 & $  0.00^{+ 0.32}_{-0.00}$ & $ 0.90^{+9.10}_{-0.48}$ & $38.29^{+1.21}_{-0.06}$ & $  1.48$ & $   1$ \\
NGC3628 & 11 20 10.41 & +13 39 34.14 & $  0.00^{+ 0.00}_{-0.00}$ & $ 1.25^{+0.13}_{-0.09}$ & $39.60^{+0.03}_{-0.02}$ & $115.86$ & $  40$ \\
NGC3628 & 11 20  9.66 & +13 37 13.09 & $  0.14^{+ 0.55}_{-0.13}$ & $ 1.18^{+1.86}_{-0.50}$ & $38.51^{+0.36}_{-0.08}$ & $  5.43$ & $   2$ \\
NGC3628 & 11 20  6.94 & +13 34 54.56 & $  0.00^{+ 0.02}_{-0.00}$ & $ 1.18^{+0.49}_{-0.28}$ & $38.57^{+0.11}_{-0.10}$ & $ 16.75$ & $   3$ \\
NGC3628 & 11 20 33.50 & +13 35 25.42 & $  0.00^{+ 0.18}_{-0.00}$ & $ 4.63^{+5.37}_{-2.83}$ & $38.94^{+0.46}_{-0.42}$ & $  2.59$ & $   3$ \\
NGC3628 & 11 20 11.82 & +13 31 22.55 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.52^{+0.07}_{-0.05}$ & $39.11^{+0.01}_{-0.01}$ & $119.45$ & $  27$ \\
NGC4125 & 12  8 17.91 & +65 11 19.37 & $  0.27^{+ 0.33}_{-0.24}$ & $ 0.50^{+0.50}_{-0.18}$ & $39.13^{+0.43}_{-0.25}$ & $  0.00$ & $   1$ \\
NGC4125 & 12  8 17.45 & +65 11 25.28 & $  0.00^{+ 0.20}_{-0.00}$ & $ 2.37^{+3.28}_{-0.89}$ & $39.49^{+0.42}_{-0.15}$ & $  1.51$ & $   2$ \\
NGC4125 & 12  8  7.53 & +65 10 28.46 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.77^{+0.08}_{-0.04}$ & $40.10^{+0.02}_{-0.01}$ & $113.59$ & $  42$ \\
NGC4125 & 12  8  7.26 & +65 11 49.05 & $  0.00^{+ 0.02}_{-0.00}$ & $ 0.90^{+0.25}_{-0.16}$ & $39.24^{+0.05}_{-0.05}$ & $ 13.70$ & $   4$ \\
NGC4125 & 12  8  1.73 & +65 10 34.66 & $  0.00^{+ 0.15}_{-0.00}$ & $ 1.18^{+1.71}_{-0.43}$ & $39.12^{+0.37}_{-0.12}$ & $  4.00$ & $   2$ \\
NGC4125 & 12  7 56.90 & +65  7 15.90 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.46^{+0.14}_{-0.11}$ & $39.02^{+0.12}_{-0.00}$ & $  2.29$ & $   3$ \\
NGC4125 & 12  7 35.74 & +65 10 22.69 & $  0.00^{+ 0.04}_{-0.00}$ & $ 0.62^{+0.24}_{-0.12}$ & $39.21^{+0.07}_{-0.02}$ & $  5.06$ & $   4$ \\
NGC4125 & 12  8 11.51 & +65  6 10.03 & $  0.00^{+ 0.22}_{-0.00}$ & $ 0.74^{+1.82}_{-0.35}$ & $39.03^{+0.50}_{-0.04}$ & $  7.02$ & $   1$ \\
NGC4365 & 12 24 29.72 & + 7 19  4.07 & $  0.00^{+ 0.13}_{-0.00}$ & $ 9.76^{+0.24}_{-8.60}$ & $40.04^{+0.08}_{-1.04}$ & $  2.20$ & $   2$ \\
NGC4365 & 12 24 28.50 & + 7 18 31.09 & $  0.00^{+ 0.17}_{-0.00}$ & $ 0.43^{+0.27}_{-0.16}$ & $38.98^{+0.34}_{-0.00}$ & $  1.53$ & $   1$ \\
NGC4365 & 12 24 27.74 & + 7 18  6.87 & $  0.01^{+ 0.34}_{-0.01}$ & $ 0.29^{+0.13}_{-0.14}$ & $38.98^{+1.14}_{-0.07}$ & $  1.54$ & $   2$ \\
NGC4365 & 12 24 26.39 & + 7 16 53.18 & $  0.03^{+ 0.28}_{-0.03}$ & $ 2.24^{+1.95}_{-0.75}$ & $39.82^{+0.27}_{-0.12}$ & $  3.34$ & $   5$ \\
NGC4365 & 12 24 25.68 & + 7 17 46.01 & $  0.36^{+ 0.41}_{-0.32}$ & $ 0.29^{+0.24}_{-0.11}$ & $39.39^{+0.88}_{-0.50}$ & $  3.30$ & $   2$ \\
NGC4365 & 12 24 20.18 & + 7 17 39.42 & $  0.00^{+ 0.25}_{-0.00}$ & $ 0.85^{+1.86}_{-0.41}$ & $38.95^{+0.48}_{-0.04}$ & $  0.95$ & $   2$ \\
NGC4365 & 12 24 14.75 & + 7 20  4.77 & $  0.00^{+ 0.03}_{-0.00}$ & $ 0.40^{+0.09}_{-0.06}$ & $39.23^{+0.08}_{-0.01}$ & $  6.48$ & $   3$ \\
NGC4365 & 12 24 38.29 & + 7 21  7.01 & $  0.00^{+ 0.13}_{-0.00}$ & $ 0.36^{+0.08}_{-0.10}$ & $39.13^{+0.33}_{-0.02}$ & $  1.27$ & $   3$ \\
NGC4365 & 12 24 14.61 & + 7 15 35.15 & $  0.00^{+ 0.07}_{-0.00}$ & $ 1.09^{+0.30}_{-0.23}$ & $39.48^{+0.05}_{-0.03}$ & $ 14.08$ & $   3$ \\
NGC4374 & 12 25 15.09 & +12 56  2.70 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.77^{+0.10}_{-0.09}$ & $39.69^{+0.03}_{-0.02}$ & $ 33.64$ & $  15$ \\
NGC4374 & 12 25  5.38 & +12 53 45.39 & $  0.00^{+ 0.15}_{-0.00}$ & $ 0.74^{+1.11}_{-0.28}$ & $38.88^{+0.32}_{-0.03}$ & $  4.24$ & $   2$ \\
NGC4374 & 12 25  1.58 & +12 52 35.93 & $  0.20^{+ 0.37}_{-0.18}$ & $ 0.39^{+0.36}_{-0.16}$ & $39.10^{+0.67}_{-0.22}$ & $  0.45$ & $   2$ \\
NGC4374 & 12 24 46.91 & +12 54 35.00 & $  0.04^{+ 0.22}_{-0.04}$ & $ 0.48^{+0.48}_{-0.20}$ & $39.23^{+0.42}_{-0.06}$ & $  2.29$ & $   3$ \\
NGC4449 & 12 28 13.26 & +44  6 55.82 & $  0.03^{+ 0.11}_{-0.02}$ & $ 0.61^{+0.24}_{-0.17}$ & $38.20^{+0.12}_{-0.04}$ & $  4.49$ & $   7$ \\
NGC4449 & 12 28 11.98 & +44  6 41.46 & $  0.03^{+ 0.18}_{-0.03}$ & $ 0.50^{+0.20}_{-0.15}$ & $38.05^{+0.26}_{-0.03}$ & $  7.10$ & $   4$ \\
NGC4449 & 12 28 11.19 & +44  6 38.52 & $  0.16^{+ 0.27}_{-0.15}$ & $ 0.32^{+0.20}_{-0.11}$ & $38.01^{+0.62}_{-0.28}$ & $  0.79$ & $   1$ \\
NGC4449 & 12 28 10.95 & +44  6 48.48 & $  0.02^{+ 0.04}_{-0.02}$ & $ 0.70^{+0.07}_{-0.06}$ & $38.83^{+0.03}_{-0.02}$ & $140.95$ & $  36$ \\
NGC4449 & 12 28 10.93 & +44  3 37.99 & $  0.09^{+ 0.05}_{-0.04}$ & $ 0.10^{+0.02}_{-0.01}$ & $39.42^{+0.40}_{-0.32}$ & $ 15.36$ & $  12$ \\
NGC4449 & 12 28  9.71 & +44  5 53.11 & $  0.07^{+ 0.15}_{-0.07}$ & $ 1.72^{+8.28}_{-0.71}$ & $38.38^{+0.88}_{-0.12}$ & $  3.49$ & $   5$ \\
NGC4449 & 12 28  9.31 & +44  5  8.27 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.61^{+0.03}_{-0.03}$ & $38.82^{+0.01}_{-0.01}$ & $ 55.28$ & $  43$ \\
NGC4449 & 12 28  7.34 & +44  4 53.79 & $  0.00^{+ 0.10}_{-0.00}$ & $ 0.31^{+0.06}_{-0.08}$ & $37.92^{+0.32}_{-0.02}$ & $  6.98$ & $   3$ \\
NGC4449 & 12 28  7.28 & +44  7 21.57 & $  0.00^{+ 0.32}_{-0.00}$ & $ 1.76^{+8.24}_{-0.91}$ & $37.92^{+0.87}_{-0.19}$ & $  0.18$ & $   1$ \\
NGC4449 & 12 28  3.88 & +44  5 43.84 & $  0.00^{+ 0.12}_{-0.00}$ & $ 1.06^{+0.88}_{-0.36}$ & $37.94^{+0.27}_{-0.05}$ & $  1.96$ & $   2$ \\
NGC4449 & 12 28  2.07 & +44  8  7.95 & $  0.38^{+ 0.33}_{-0.31}$ & $ 0.48^{+0.58}_{-0.16}$ & $38.22^{+0.41}_{-0.22}$ & $  4.76$ & $   2$ \\
NGC4485 & 12 30 49.60 & +41 40 56.74 & $  0.00^{+ 0.02}_{-0.00}$ & $ 1.03^{+0.22}_{-0.18}$ & $39.14^{+0.04}_{-0.04}$ & $ 20.51$ & $   7$ \\
NGC4485 & 12 30 40.42 & +41 38 13.42 & $  0.33^{+ 0.43}_{-0.30}$ & $ 1.45^{+4.29}_{-0.56}$ & $38.97^{+0.53}_{-0.10}$ & $  0.69$ & $   3$ \\
NGC4485 & 12 30 36.33 & +41 38 37.78 & $  0.16^{+ 0.09}_{-0.09}$ & $ 1.64^{+0.35}_{-0.22}$ & $39.68^{+0.05}_{-0.04}$ & $ 28.49$ & $  22$ \\
NGC4485 & 12 30 34.45 & +41 38 49.86 & $  0.17^{+ 0.45}_{-0.16}$ & $ 0.87^{+0.76}_{-0.31}$ & $38.91^{+0.21}_{-0.08}$ & $  1.56$ & $   2$ \\
NGC4485 & 12 30 32.27 & +41 39 18.07 & $  0.17^{+ 0.09}_{-0.09}$ & $ 1.60^{+0.39}_{-0.25}$ & $39.66^{+0.06}_{-0.04}$ & $ 18.25$ & $  21$ \\
NGC4485 & 12 30 30.82 & +41 39 11.48 & $  0.41^{+ 0.15}_{-0.13}$ & $ 1.72^{+0.32}_{-0.27}$ & $39.89^{+0.04}_{-0.03}$ & $ 25.31$ & $  29$ \\
NGC4485 & 12 30 30.40 & +41 38 52.86 & $  0.13^{+ 0.31}_{-0.11}$ & $ 1.72^{+1.13}_{-0.49}$ & $39.11^{+0.18}_{-0.08}$ & $  1.73$ & $   4$ \\
NGC4485 & 12 30 29.55 & +41 39 27.61 & $  1.84^{+ 0.60}_{-0.51}$ & $ 0.85^{+0.18}_{-0.11}$ & $39.80^{+0.15}_{-0.12}$ & $  9.99$ & $  10$ \\
NGC4485 & 12 30 25.30 & +41 39 24.74 & $  0.12^{+ 0.60}_{-0.11}$ & $ 1.28^{+3.22}_{-0.58}$ & $38.62^{+0.51}_{-0.10}$ & $  2.84$ & $   2$ \\
NGC4559 & 12 35 57.79 & +27 58  7.43 & $  0.13^{+ 0.11}_{-0.11}$ & $ 0.94^{+0.38}_{-0.22}$ & $39.63^{+0.05}_{-0.06}$ & $  9.73$ & $   7$ \\
NGC4579 & 12 37 53.89 & +11 50 20.33 & $  0.00^{+ 0.10}_{-0.00}$ & $ 1.09^{+0.72}_{-0.38}$ & $39.42^{+0.20}_{-0.08}$ & $  2.66$ & $   3$ \\
NGC4579 & 12 37 44.13 & +11 49 17.32 & $  0.00^{+ 0.13}_{-0.00}$ & $ 2.03^{+4.14}_{-0.72}$ & $39.31^{+0.52}_{-0.19}$ & $  3.77$ & $   3$ \\
NGC4579 & 12 37 40.30 & +11 47 27.48 & $  0.02^{+ 0.02}_{-0.02}$ & $ 1.35^{+0.10}_{-0.09}$ & $40.56^{+0.02}_{-0.02}$ & $ 65.02$ & $  63$ \\
NGC4594 & 12 40  7.06 & -11 37 53.49 & $  0.00^{+ 0.35}_{-0.00}$ & $ 1.41^{+8.59}_{-0.71}$ & $38.67^{+0.98}_{-0.17}$ & $  3.14$ & $   1$ \\
NGC4594 & 12 40  2.01 & -11 39 40.56 & $  0.46^{+ 1.25}_{-0.43}$ & $ 0.08^{+0.12}_{-0.04}$ & $41.27^{+5.88}_{-2.37}$ & $  1.67$ & $   2$ \\
NGC4594 & 12 40  1.09 & -11 37 24.13 & $  0.05^{+ 0.04}_{-0.04}$ & $ 0.26^{+0.03}_{-0.03}$ & $39.58^{+0.14}_{-0.12}$ & $ 16.78$ & $  17$ \\
NGC4594 & 12 40  0.97 & -11 36 54.20 & $  0.00^{+ 0.08}_{-0.00}$ & $ 0.79^{+0.21}_{-0.18}$ & $39.25^{+0.06}_{-0.03}$ & $  4.47$ & $   9$ \\
NGC4594 & 12 40  0.71 & -11 35 19.74 & $  0.00^{+ 0.12}_{-0.00}$ & $ 2.02^{+2.47}_{-0.63}$ & $39.04^{+0.36}_{-0.18}$ & $  1.51$ & $   2$ \\
NGC4594 & 12 40  0.38 & -11 37 23.70 & $  0.00^{+ 0.07}_{-0.00}$ & $ 0.55^{+0.27}_{-0.15}$ & $38.70^{+0.09}_{-0.01}$ & $  3.67$ & $   2$ \\
NGC4594 & 12 40  0.07 & -11 37  8.75 & $  0.18^{+ 0.46}_{-0.16}$ & $ 0.86^{+0.73}_{-0.34}$ & $38.81^{+0.26}_{-0.10}$ & $  0.00$ & $   1$ \\
NGC4594 & 12 39 59.93 & -11 36 23.27 & $  0.00^{+ 0.25}_{-0.00}$ & $ 2.16^{+7.84}_{-1.40}$ & $39.11^{+0.87}_{-0.32}$ & $  7.75$ & $   1$ \\
NGC4594 & 12 39 59.10 & -11 37 19.78 & $  0.12^{+ 0.39}_{-0.12}$ & $ 0.30^{+0.29}_{-0.14}$ & $38.89^{+1.07}_{-0.24}$ & $  0.02$ & $   1$ \\
NGC4594 & 12 39 57.41 & -11 37 20.07 & $  0.00^{+ 0.08}_{-0.00}$ & $ 1.97^{+8.03}_{-0.74}$ & $39.16^{+0.86}_{-0.19}$ & $  8.39$ & $   2$ \\
NGC4594 & 12 39 51.98 & -11 35 52.18 & $  0.00^{+ 0.32}_{-0.00}$ & $ 0.46^{+0.74}_{-0.20}$ & $38.64^{+0.54}_{-0.00}$ & $  2.57$ & $   1$ \\
NGC4594 & 12 39 50.96 & -11 38 23.63 & $  0.62^{+ 0.62}_{-0.52}$ & $ 0.75^{+0.54}_{-0.24}$ & $39.15^{+0.31}_{-0.20}$ & $  0.27$ & $   1$ \\
NGC4594 & 12 39 48.62 & -11 37 13.33 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.79^{+0.21}_{-0.15}$ & $39.02^{+0.05}_{-0.03}$ & $  4.53$ & $   4$ \\
NGC4594 & 12 39 45.22 & -11 38 49.81 & $  0.22^{+ 0.06}_{-0.06}$ & $ 0.21^{+0.03}_{-0.02}$ & $40.28^{+0.19}_{-0.19}$ & $104.94$ & $  26$ \\
NGC4594 & 12 40 10.46 & -11 36 39.07 & $  0.00^{+ 0.08}_{-0.00}$ & $ 1.45^{+1.78}_{-0.48}$ & $38.93^{+0.35}_{-0.12}$ & $  7.60$ & $   2$ \\
NGC4594 & 12 39 59.04 & -11 35 12.01 & $  0.33^{+ 0.34}_{-0.29}$ & $ 0.91^{+0.89}_{-0.30}$ & $39.00^{+0.17}_{-0.14}$ & $  1.52$ & $   2$ \\
NGC4594 & 12 39 45.27 & -11 36  0.63 & $  0.06^{+ 0.26}_{-0.06}$ & $ 1.17^{+1.15}_{-0.42}$ & $38.92^{+0.22}_{-0.09}$ & $  2.42$ & $   2$ \\
NGC4594 & 12 39 43.63 & -11 40 34.08 & $  0.00^{+ 0.19}_{-0.00}$ & $ 0.91^{+0.35}_{-0.24}$ & $39.02^{+0.08}_{-0.02}$ & $  8.45$ & $   3$ \\
NGC4631 & 12 42 11.13 & +32 32 35.94 & $  2.82^{+ 0.25}_{-0.23}$ & $ 1.28^{+0.13}_{-0.12}$ & $39.99^{+0.04}_{-0.03}$ & $ 43.86$ & $  48$ \\
NGC4631 & 12 42  7.37 & +32 32 33.82 & $  0.34^{+ 0.54}_{-0.30}$ & $ 1.49^{+1.17}_{-0.43}$ & $38.86^{+0.15}_{-0.07}$ & $  3.33$ & $   5$ \\
NGC4631 & 12 42  6.61 & +32 32  8.44 & $  1.66^{+ 1.97}_{-1.51}$ & $ 0.87^{+8.89}_{-0.37}$ & $38.65^{+0.61}_{-0.26}$ & $  0.61$ & $   1$ \\
NGC4631 & 12 42  6.18 & +32 31 53.08 & $  0.32^{+ 1.10}_{-0.27}$ & $ 6.02^{+3.98}_{-5.04}$ & $38.77^{+0.39}_{-0.62}$ & $  1.88$ & $   1$ \\
NGC4631 & 12 42  6.13 & +32 32 46.64 & $  0.16^{+ 0.12}_{-0.11}$ & $ 1.49^{+0.70}_{-0.37}$ & $38.96^{+0.11}_{-0.06}$ & $ 22.33$ & $  13$ \\
NGC4631 & 12 42  5.48 & +32 30 37.39 & $  0.13^{+ 0.45}_{-0.13}$ & $ 0.62^{+9.38}_{-0.33}$ & $37.82^{+1.15}_{-0.19}$ & $  0.01$ & $   1$ \\
NGC4631 & 12 42  5.00 & +32 31 52.15 & $  0.86^{+ 1.03}_{-0.79}$ & $ 1.72^{+8.28}_{-0.86}$ & $38.49^{+0.79}_{-0.15}$ & $  6.71$ & $   1$ \\
NGC4631 & 12 42  4.04 & +32 34  8.51 & $  0.00^{+ 0.46}_{-0.00}$ & $ 3.46^{+6.54}_{-2.94}$ & $38.87^{+0.68}_{-0.62}$ & $  1.32$ & $   1$ \\
NGC4631 & 12 42  0.11 & +32 31 58.99 & $  0.00^{+ 0.02}_{-0.00}$ & $ 0.81^{+0.15}_{-0.09}$ & $38.55^{+0.04}_{-0.02}$ & $ 16.12$ & $  12$ \\
NGC4631 & 12 41 58.02 & +32 28 51.28 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.25^{+0.09}_{-0.12}$ & $39.14^{+0.03}_{-0.03}$ & $ 32.43$ & $  36$ \\
NGC4631 & 12 41 57.41 & +32 32  3.11 & $  0.11^{+ 0.48}_{-0.11}$ & $ 0.43^{+0.76}_{-0.22}$ & $38.05^{+0.89}_{-0.12}$ & $  9.02$ & $   1$ \\
NGC4631 & 12 41 55.98 & +32 30 44.88 & $  0.07^{+ 3.82}_{-0.05}$ & $10.00^{+0.00}_{-8.86}$ & $39.37^{+0.11}_{-0.72}$ & $  0.39$ & $   1$ \\
NGC4649 & 12 43 48.62 & +11 32 40.96 & $  0.00^{+ 0.17}_{-0.00}$ & $ 0.44^{+0.29}_{-0.18}$ & $38.66^{+0.38}_{-0.00}$ & $  0.51$ & $   2$ \\
NGC4649 & 12 43 47.03 & +11 32 36.75 & $  0.00^{+ 0.04}_{-0.00}$ & $ 1.64^{+0.70}_{-0.39}$ & $39.37^{+0.14}_{-0.11}$ & $  5.79$ & $   4$ \\
NGC4649 & 12 43 46.91 & +11 32 33.85 & $  0.00^{+ 0.07}_{-0.00}$ & $ 0.70^{+1.02}_{-0.27}$ & $38.73^{+0.34}_{-0.07}$ & $  2.73$ & $   1$ \\
NGC4649 & 12 43 45.00 & +11 32 33.33 & $  0.00^{+ 0.05}_{-0.00}$ & $ 1.01^{+0.55}_{-0.31}$ & $39.16^{+0.14}_{-0.09}$ & $  8.21$ & $   3$ \\
NGC4649 & 12 43 44.56 & +11 31 50.74 & $  0.00^{+ 0.22}_{-0.00}$ & $ 1.72^{+8.28}_{-0.78}$ & $39.07^{+0.90}_{-0.19}$ & $ 10.13$ & $   1$ \\
NGC4649 & 12 43 43.59 & +11 33  2.66 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.61^{+0.33}_{-0.15}$ & $38.77^{+0.07}_{-0.00}$ & $  5.65$ & $   2$ \\
NGC4649 & 12 43 41.77 & +11 34 33.78 & $  0.00^{+ 0.10}_{-0.00}$ & $ 0.49^{+0.28}_{-0.16}$ & $39.01^{+0.18}_{-0.00}$ & $  1.87$ & $   2$ \\
NGC4649 & 12 43 40.46 & +11 32 43.01 & $  0.00^{+ 0.06}_{-0.00}$ & $ 0.62^{+0.35}_{-0.16}$ & $38.98^{+0.09}_{-0.01}$ & $  5.78$ & $   2$ \\
NGC4649 & 12 43 38.07 & +11 32 41.74 & $  0.00^{+ 0.20}_{-0.00}$ & $ 1.93^{+8.07}_{-1.33}$ & $38.93^{+0.94}_{-0.37}$ & $  0.02$ & $   2$ \\
NGC4649 & 12 43 37.94 & +11 34 35.22 & $  0.00^{+ 0.12}_{-0.00}$ & $ 1.59^{+8.41}_{-0.67}$ & $38.90^{+0.91}_{-0.17}$ & $  4.28$ & $   2$ \\
NGC4649 & 12 43 37.84 & +11 33 28.36 & $  0.00^{+ 0.13}_{-0.00}$ & $ 1.13^{+0.87}_{-0.37}$ & $38.83^{+0.20}_{-0.06}$ & $  1.99$ & $   3$ \\
NGC4649 & 12 43 37.27 & +11 31 43.68 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.67^{+0.12}_{-0.14}$ & $39.28^{+0.02}_{-0.03}$ & $ 37.35$ & $   8$ \\
NGC4649 & 12 43 36.49 & +11 30  8.96 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.40^{+0.11}_{-0.05}$ & $40.20^{+0.02}_{-0.04}$ & $ 64.29$ & $  13$ \\
NGC4649 & 12 43 35.48 & +11 34 27.30 & $  0.00^{+ 0.24}_{-0.00}$ & $ 0.77^{+1.10}_{-0.38}$ & $38.85^{+0.33}_{-0.05}$ & $  8.09$ & $   1$ \\
NGC4649 & 12 43 34.79 & +11 32 27.49 & $  0.00^{+ 0.16}_{-0.00}$ & $ 0.86^{+0.36}_{-0.26}$ & $38.82^{+0.13}_{-0.00}$ & $  7.38$ & $   3$ \\
NGC4649 & 12 43 34.04 & +11 33 41.88 & $  0.00^{+ 0.08}_{-0.00}$ & $ 1.09^{+0.58}_{-0.33}$ & $39.18^{+0.15}_{-0.08}$ & $  1.20$ & $   3$ \\
NGC4649 & 12 43 33.94 & +11 34  1.24 & $  0.00^{+ 0.19}_{-0.00}$ & $ 1.56^{+8.44}_{-1.02}$ & $39.01^{+1.05}_{-0.27}$ & $  1.04$ & $   2$ \\
NGC4649 & 12 43 33.30 & +11 32 39.86 & $  0.00^{+ 0.08}_{-0.00}$ & $ 1.94^{+8.06}_{-0.77}$ & $39.28^{+0.85}_{-0.21}$ & $  2.13$ & $   3$ \\
NGC4649 & 12 43 32.64 & +11 30  2.04 & $  0.00^{+ 0.13}_{-0.00}$ & $ 0.87^{+0.29}_{-0.22}$ & $39.18^{+0.07}_{-0.02}$ & $  5.34$ & $   2$ \\
NGC4649 & 12 43 32.08 & +11 34 18.57 & $  0.00^{+ 0.65}_{-0.00}$ & $ 2.05^{+7.95}_{-1.16}$ & $39.41^{+0.84}_{-0.21}$ & $  0.64$ & $   2$ \\
NGC4649 & 12 43 32.03 & +11 31 46.64 & $  0.00^{+ 0.06}_{-0.00}$ & $ 1.02^{+1.43}_{-0.37}$ & $38.95^{+0.31}_{-0.09}$ & $ 12.18$ & $   2$ \\
NGC4649 & 12 43 29.87 & +11 33 18.25 & $  0.00^{+ 0.17}_{-0.00}$ & $ 1.95^{+8.05}_{-0.92}$ & $39.12^{+0.85}_{-0.22}$ & $  1.46$ & $   1$ \\
NGC4649 & 12 43 55.01 & +11 33  7.98 & $  0.00^{+ 0.07}_{-0.00}$ & $ 0.62^{+0.34}_{-0.19}$ & $39.03^{+0.13}_{-0.04}$ & $  4.68$ & $   3$ \\
NGC4697 & 12 48 47.49 &  -5 45 13.03 & $  0.00^{+ 0.25}_{-0.00}$ & $ 0.70^{+1.59}_{-0.32}$ & $39.06^{+0.43}_{-0.02}$ & $  1.00$ & $   1$ \\
NGC4697 & 12 48 46.84 &  -5 48 53.64 & $  0.00^{+ 0.02}_{-0.00}$ & $ 1.41^{+0.67}_{-0.30}$ & $39.25^{+0.18}_{-0.09}$ & $ 32.92$ & $  11$ \\
NGC4697 & 12 48 45.44 &  -5 45 42.64 & $  0.03^{+ 0.22}_{-0.03}$ & $ 0.35^{+0.16}_{-0.14}$ & $38.57^{+0.57}_{-0.07}$ & $  1.85$ & $   1$ \\
NGC4697 & 12 48 39.36 &  -5 47 30.62 & $  0.00^{+ 0.19}_{-0.00}$ & $ 0.99^{+2.39}_{-0.47}$ & $38.45^{+0.54}_{-0.11}$ & $  0.67$ & $   2$ \\
NGC4697 & 12 48 39.31 &  -5 48  7.54 & $  0.00^{+ 0.04}_{-0.00}$ & $ 1.06^{+0.46}_{-0.23}$ & $38.94^{+0.14}_{-0.06}$ & $  2.98$ & $   5$ \\
NGC4697 & 12 48 37.50 &  -5 47 43.71 & $  0.00^{+ 0.11}_{-0.00}$ & $ 0.74^{+1.56}_{-0.33}$ & $38.31^{+0.47}_{-0.08}$ & $  2.16$ & $   2$ \\
NGC4697 & 12 48 36.96 &  -5 48  1.38 & $  0.00^{+ 0.12}_{-0.00}$ & $ 0.92^{+9.08}_{-0.44}$ & $38.40^{+1.24}_{-0.10}$ & $  2.81$ & $   2$ \\
NGC4697 & 12 48 36.71 &  -5 47 32.10 & $  0.05^{+ 0.20}_{-0.05}$ & $ 1.32^{+3.65}_{-0.58}$ & $38.87^{+0.61}_{-0.12}$ & $  0.02$ & $   2$ \\
NGC4697 & 12 48 35.97 &  -5 47 56.88 & $  0.00^{+ 0.09}_{-0.00}$ & $ 1.49^{+1.30}_{-0.50}$ & $38.63^{+0.24}_{-0.13}$ & $  1.85$ & $   3$ \\
NGC4697 & 12 48 35.92 &  -5 47 52.58 & $  0.00^{+ 0.24}_{-0.00}$ & $ 2.72^{+7.28}_{-1.96}$ & $38.88^{+0.79}_{-0.42}$ & $  0.79$ & $   2$ \\
NGC4697 & 12 48 34.53 &  -5 47 49.74 & $  0.31^{+ 0.75}_{-0.31}$ & $ 0.08^{+0.15}_{-0.04}$ & $40.21^{+3.93}_{-1.78}$ & $  2.23$ & $   1$ \\
NGC4697 & 12 48 34.49 &  -5 47 40.36 & $  0.00^{+ 0.11}_{-0.00}$ & $ 5.47^{+4.53}_{-4.02}$ & $39.27^{+0.38}_{-0.63}$ & $  0.96$ & $   1$ \\
NGC4697 & 12 48 33.19 &  -5 47 42.15 & $  0.00^{+ 0.04}_{-0.00}$ & $ 1.32^{+0.40}_{-0.28}$ & $39.02^{+0.12}_{-0.07}$ & $  1.92$ & $   6$ \\
NGC4697 & 12 48 30.81 &  -5 48 37.29 & $  0.01^{+ 0.16}_{-0.01}$ & $ 0.83^{+0.73}_{-0.37}$ & $38.55^{+0.22}_{-0.06}$ & $  0.31$ & $   1$ \\
NGC4697 & 12 48 27.33 &  -5 47  8.08 & $  0.03^{+ 0.28}_{-0.02}$ & $ 0.87^{+0.80}_{-0.38}$ & $38.68^{+0.21}_{-0.06}$ & $  0.29$ & $   1$ \\
NGC4697 & 12 48 24.44 &  -5 45 58.06 & $  0.53^{+ 0.10}_{-0.14}$ & $ 1.85^{+0.56}_{-0.25}$ & $39.85^{+0.09}_{-0.03}$ & $ 27.93$ & $  20$ \\
NGC4697 & 12 48 23.73 &  -5 46 59.79 & $  0.00^{+ 0.20}_{-0.00}$ & $ 0.85^{+1.80}_{-0.39}$ & $38.30^{+0.47}_{-0.07}$ & $  2.18$ & $   1$ \\
NGC4697 & 12 48 27.01 &  -5 49 26.02 & $  0.22^{+ 0.35}_{-0.21}$ & $ 0.44^{+2.93}_{-0.20}$ & $38.65^{+0.65}_{-0.22}$ & $  0.03$ & $   1$ \\
NGC4697 & 12 48 22.45 &  -5 48 15.38 & $  0.00^{+ 0.09}_{-0.00}$ & $ 0.77^{+2.68}_{-0.31}$ & $38.39^{+0.68}_{-0.06}$ & $  2.47$ & $   2$ \\
NGC5055 & 13 16  2.27 & +42  1 53.65 & $  0.28^{+ 0.06}_{-0.09}$ & $ 0.51^{+0.08}_{-0.06}$ & $39.64^{+0.07}_{-0.08}$ & $ 23.14$ & $  22$ \\
NGC5055 & 13 15 53.89 & +42  1  4.70 & $  0.20^{+ 0.40}_{-0.18}$ & $ 1.75^{+1.66}_{-0.58}$ & $39.11^{+0.20}_{-0.11}$ & $  1.72$ & $   3$ \\
NGC5055 & 13 15 53.25 & +42  2 14.84 & $  0.00^{+ 0.04}_{-0.00}$ & $ 1.03^{+0.20}_{-0.15}$ & $39.07^{+0.05}_{-0.03}$ & $ 11.42$ & $   9$ \\
NGC5055 & 13 15 51.39 & +42  1 40.42 & $  0.07^{+ 0.10}_{-0.07}$ & $ 0.16^{+0.05}_{-0.04}$ & $39.42^{+0.52}_{-0.34}$ & $  4.84$ & $   7$ \\
NGC5055 & 13 15 50.93 & +42  2  0.17 & $  0.11^{+ 0.35}_{-0.11}$ & $ 1.68^{+8.32}_{-1.00}$ & $38.91^{+0.94}_{-0.21}$ & $  0.80$ & $   1$ \\
NGC5055 & 13 15 50.04 & +42  2 15.40 & $  0.46^{+ 0.50}_{-0.44}$ & $ 0.44^{+0.92}_{-0.18}$ & $38.83^{+0.68}_{-0.32}$ & $  2.09$ & $   1$ \\
NGC5055 & 13 15 49.57 & +42  1 27.09 & $  0.51^{+ 0.69}_{-0.44}$ & $10.00^{+0.00}_{-7.51}$ & $40.01^{+0.07}_{-0.62}$ & $  1.83$ & $   2$ \\
NGC5055 & 13 15 49.47 & +41 59 51.75 & $  0.00^{+ 0.32}_{-0.00}$ & $ 1.21^{+2.45}_{-0.50}$ & $38.57^{+0.48}_{-0.07}$ & $  4.11$ & $   2$ \\
NGC5055 & 13 15 47.81 & +42  1 24.99 & $  0.56^{+ 0.64}_{-0.50}$ & $ 1.70^{+4.43}_{-0.66}$ & $38.98^{+0.46}_{-0.13}$ & $  5.56$ & $   2$ \\
NGC5055 & 13 15 46.64 & +42  2  0.96 & $  0.51^{+ 0.25}_{-0.38}$ & $ 0.11^{+0.08}_{-0.02}$ & $40.62^{+0.98}_{-1.49}$ & $  9.75$ & $   4$ \\
NGC5055 & 13 15 43.86 & +41 59 10.34 & $  0.00^{+ 0.13}_{-0.00}$ & $ 0.70^{+0.48}_{-0.24}$ & $38.55^{+0.12}_{-0.03}$ & $  1.46$ & $   2$ \\
NGC5055 & 13 15 40.85 & +42  1 49.29 & $  0.00^{+ 0.05}_{-0.00}$ & $ 1.10^{+0.27}_{-0.20}$ & $39.07^{+0.07}_{-0.04}$ & $  9.29$ & $   9$ \\
NGC5055 & 13 15 39.71 & +42  1 10.97 & $  0.02^{+ 0.16}_{-0.02}$ & $ 0.78^{+0.24}_{-0.20}$ & $38.92^{+0.10}_{-0.03}$ & $  4.77$ & $   5$ \\
NGC5055 & 13 15 39.49 & +42  2 26.57 & $  1.73^{+ 1.67}_{-1.30}$ & $ 0.59^{+1.09}_{-0.24}$ & $39.22^{+0.83}_{-0.40}$ & $  5.35$ & $   2$ \\
NGC5055 & 13 15 39.32 & +42  1 53.38 & $  0.15^{+ 0.33}_{-0.14}$ & $ 1.20^{+0.67}_{-0.32}$ & $39.07^{+0.08}_{-0.07}$ & $  3.25$ & $   4$ \\
NGC5055 & 13 15 30.18 & +42  3 13.48 & $  1.09^{+ 0.33}_{-0.27}$ & $ 0.07^{+0.02}_{-0.01}$ & $43.51^{+1.41}_{-1.17}$ & $ 58.58$ & $  11$ \\
NGC5128 & 13 25 58.80 & -43  4 31.27 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.34^{+0.15}_{-0.11}$ & $38.90^{+0.03}_{-0.02}$ & $ 47.68$ & $  29$ \\
NGC5128 & 13 25 44.08 & -43  6 10.97 & $  0.00^{+ 0.36}_{-0.00}$ & $ 1.85^{+1.21}_{-0.59}$ & $38.24^{+0.19}_{-0.11}$ & $  6.29$ & $   2$ \\
NGC5128 & 13 25 40.64 & -43  1 15.49 & $  0.00^{+ 0.18}_{-0.00}$ & $ 1.38^{+8.62}_{-0.34}$ & $38.09^{+1.08}_{-0.08}$ & $  1.86$ & $   2$ \\
NGC5128 & 13 25 38.38 & -43  2  6.36 & $  0.54^{+ 0.28}_{-0.26}$ & $ 2.44^{+1.82}_{-0.66}$ & $39.04^{+0.20}_{-0.10}$ & $ 10.81$ & $  16$ \\
NGC5128 & 13 25 36.71 & -43  0 58.14 & $  0.00^{+ 0.36}_{-0.00}$ & $ 2.20^{+6.60}_{-0.97}$ & $38.04^{+0.67}_{-0.18}$ & $  2.46$ & $   3$ \\
NGC5128 & 13 25 33.43 & -43  0 53.11 & $  0.09^{+ 0.57}_{-0.09}$ & $ 1.85^{+8.15}_{-0.89}$ & $38.16^{+0.80}_{-0.16}$ & $  1.69$ & $   2$ \\
NGC5128 & 13 25 32.53 & -43  1 34.82 & $  0.46^{+ 0.94}_{-0.42}$ & $10.00^{+0.00}_{-7.63}$ & $39.23^{+0.07}_{-0.64}$ & $  2.73$ & $   3$ \\
NGC5128 & 13 25 32.09 & -43  2 32.27 & $  0.00^{+ 0.28}_{-0.00}$ & $ 1.42^{+1.14}_{-0.49}$ & $38.11^{+0.23}_{-0.09}$ & $  1.31$ & $   3$ \\
NGC5128 & 13 25 31.68 & -43  0  3.65 & $  0.00^{+ 0.25}_{-0.00}$ & $ 1.79^{+0.72}_{-0.46}$ & $38.33^{+0.13}_{-0.07}$ & $  9.09$ & $   4$ \\
NGC5128 & 13 25 28.82 & -42 59 48.60 & $  0.16^{+ 0.27}_{-0.14}$ & $ 1.40^{+0.75}_{-0.36}$ & $38.38^{+0.11}_{-0.09}$ & $  5.06$ & $   5$ \\
NGC5128 & 13 25 28.28 & -43  2 54.14 & $  0.00^{+ 0.25}_{-0.00}$ & $ 0.66^{+0.27}_{-0.23}$ & $37.75^{+0.18}_{-0.01}$ & $  3.64$ & $   3$ \\
NGC5128 & 13 25 27.52 & -43  2 14.78 & $  0.00^{+ 0.10}_{-0.00}$ & $ 1.12^{+0.37}_{-0.23}$ & $38.20^{+0.08}_{-0.05}$ & $  5.92$ & $   4$ \\
NGC5128 & 13 25 27.57 & -43  1 28.85 & $  0.40^{+ 0.80}_{-0.40}$ & $ 2.12^{+7.88}_{-0.94}$ & $38.49^{+0.69}_{-0.19}$ & $  3.91$ & $   4$ \\
NGC5128 & 13 25 27.15 & -43  1 59.88 & $  0.06^{+ 0.34}_{-0.06}$ & $ 1.35^{+0.80}_{-0.45}$ & $38.22^{+0.17}_{-0.09}$ & $  0.24$ & $   3$ \\
NGC5128 & 13 25 25.84 & -43  0 56.39 & $  0.20^{+ 0.23}_{-0.18}$ & $ 1.09^{+0.37}_{-0.22}$ & $38.65^{+0.07}_{-0.06}$ & $ 16.35$ & $  12$ \\
NGC5128 & 13 25 24.28 & -42 59 59.89 & $  0.54^{+ 1.03}_{-0.49}$ & $ 2.58^{+7.42}_{-1.12}$ & $38.55^{+0.59}_{-0.13}$ & $  5.08$ & $   4$ \\
NGC5128 & 13 25 23.71 & -43  3 26.75 & $  0.00^{+ 0.25}_{-0.00}$ & $ 1.24^{+1.44}_{-0.45}$ & $37.84^{+0.31}_{-0.08}$ & $  2.79$ & $   3$ \\
NGC5128 & 13 25 23.65 & -43  2 21.10 & $  0.03^{+ 0.49}_{-0.03}$ & $ 1.17^{+1.25}_{-0.21}$ & $37.74^{+0.29}_{-0.03}$ & $  1.26$ & $   2$ \\
NGC5128 & 13 25 23.60 & -43  1 39.09 & $  0.00^{+ 0.36}_{-0.00}$ & $ 1.65^{+4.23}_{-0.75}$ & $38.17^{+0.64}_{-0.09}$ & $  0.93$ & $   2$ \\
NGC5128 & 13 25 22.94 & -43  1 25.49 & $  0.00^{+ 0.09}_{-0.00}$ & $ 2.06^{+1.74}_{-0.61}$ & $38.46^{+0.28}_{-0.14}$ & $  5.99$ & $   5$ \\
NGC5128 & 13 25 18.58 & -43  1 16.97 & $  0.00^{+ 0.77}_{-0.00}$ & $ 1.34^{+1.84}_{-0.66}$ & $37.93^{+0.33}_{-0.09}$ & $  0.27$ & $   1$ \\
NGC5128 & 13 25 24.01 & -43  0 59.68 & $  0.83^{+ 2.23}_{-0.72}$ & $ 1.30^{+2.64}_{-0.59}$ & $38.24^{+0.45}_{-0.10}$ & $  1.63$ & $   3$ \\
NGC5194 & 13 30  7.56 & +47 11  5.68 & $  0.00^{+ 0.00}_{-0.00}$ & $ 0.95^{+0.09}_{-0.06}$ & $39.52^{+0.02}_{-0.02}$ & $ 97.30$ & $  36$ \\
NGC5194 & 13 30  6.50 & +47  8 34.60 & $  0.00^{+ 0.05}_{-0.00}$ & $ 0.95^{+0.22}_{-0.16}$ & $38.87^{+0.05}_{-0.03}$ & $  4.95$ & $   5$ \\
NGC5194 & 13 30  4.33 & +47 13 20.75 & $  0.00^{+ 0.07}_{-0.00}$ & $ 2.27^{+3.29}_{-0.74}$ & $38.94^{+0.42}_{-0.15}$ & $  3.37$ & $   2$ \\
NGC5194 & 13 29 57.56 & +47 10 48.32 & $  0.01^{+ 0.07}_{-0.01}$ & $ 1.01^{+0.35}_{-0.24}$ & $39.06^{+0.09}_{-0.05}$ & $  8.76$ & $  10$ \\
NGC5194 & 13 29 56.26 & +47 14 51.49 & $  0.00^{+ 0.15}_{-0.00}$ & $ 1.15^{+1.81}_{-0.45}$ & $38.87^{+0.42}_{-0.09}$ & $  5.60$ & $   3$ \\
NGC5194 & 13 29 54.18 & +47 11 36.94 & $  0.15^{+ 0.36}_{-0.13}$ & $ 1.42^{+4.16}_{-0.57}$ & $38.60^{+0.57}_{-0.12}$ & $  3.18$ & $   3$ \\
NGC5194 & 13 29 53.79 & +47 14 31.45 & $  0.00^{+ 0.51}_{-0.00}$ & $ 0.49^{+0.54}_{-0.27}$ & $38.46^{+0.89}_{-0.00}$ & $  0.16$ & $   1$ \\
NGC5194 & 13 29 53.73 & +47 14 35.69 & $  0.00^{+ 0.02}_{-0.00}$ & $ 1.85^{+0.68}_{-0.36}$ & $39.38^{+0.14}_{-0.12}$ & $ 10.37$ & $  15$ \\
NGC5194 & 13 29 53.31 & +47 10 42.38 & $  0.00^{+ 0.01}_{-0.00}$ & $ 1.45^{+0.19}_{-0.13}$ & $39.46^{+0.04}_{-0.03}$ & $ 49.01$ & $  24$ \\
NGC5194 & 13 29 51.36 & +47 10 32.28 & $  0.00^{+ 0.14}_{-0.00}$ & $ 1.94^{+3.80}_{-0.83}$ & $39.02^{+0.56}_{-0.19}$ & $  1.74$ & $   4$ \\
NGC5194 & 13 29 50.81 & +47 10 31.20 & $  0.00^{+ 0.17}_{-0.00}$ & $ 0.96^{+9.04}_{-0.45}$ & $38.34^{+1.20}_{-0.07}$ & $  2.15$ & $   2$ \\
NGC5194 & 13 29 50.66 & +47 11 54.95 & $  3.15^{+ 0.80}_{-0.85}$ & $ 1.85^{+1.61}_{-0.50}$ & $39.86^{+0.13}_{-0.07}$ & $  9.44$ & $   9$ \\
NGC5194 & 13 29 49.03 & +47 10 53.38 & $  0.00^{+ 0.09}_{-0.00}$ & $ 1.35^{+0.68}_{-0.31}$ & $38.78^{+0.17}_{-0.05}$ & $  3.09$ & $   3$ \\
NGC5194 & 13 29 43.35 & +47 15 25.33 & $  0.00^{+ 0.13}_{-0.00}$ & $ 0.55^{+0.28}_{-0.19}$ & $38.46^{+0.19}_{-0.00}$ & $  2.23$ & $   2$ \\
NGC5194 & 13 29 43.29 & +47 11 34.65 & $  0.12^{+ 0.20}_{-0.12}$ & $ 0.14^{+0.07}_{-0.04}$ & $39.73^{+0.95}_{-0.57}$ & $  5.54$ & $   9$ \\
NGC5194 & 13 29 39.45 & +47 12 43.60 & $  0.00^{+ 0.03}_{-0.00}$ & $ 1.11^{+0.27}_{-0.20}$ & $38.92^{+0.06}_{-0.04}$ & $ 11.53$ & $   6$ \\
NGC5194 & 13 29 38.63 & +47 13 36.16 & $  0.00^{+ 0.32}_{-0.00}$ & $ 0.39^{+0.15}_{-0.16}$ & $38.39^{+0.62}_{-0.03}$ & $  2.96$ & $   1$ \\
NGC5194 & 13 30 11.02 & +47 10 40.46 & $  0.00^{+ 0.12}_{-0.00}$ & $ 1.64^{+8.36}_{-0.95}$ & $38.59^{+0.99}_{-0.28}$ & $  1.79$ & $   2$ \\
NGC5457 & 14  3 36.10 & +54 19 23.92 & $  0.00^{+ 0.13}_{-0.00}$ & $ 0.36^{+0.18}_{-0.12}$ & $38.60^{+0.36}_{-0.01}$ & $  1.66$ & $   1$ \\
NGC5457 & 14  3 32.45 & +54 21  2.04 & $  0.10^{+ 0.08}_{-0.06}$ & $ 0.09^{+0.02}_{-0.01}$ & $40.30^{+0.55}_{-0.44}$ & $  3.01$ & $   8$ \\
NGC5457 & 14  3 24.25 & +54 19 48.02 & $  0.37^{+ 0.58}_{-0.33}$ & $ 1.98^{+8.02}_{-1.11}$ & $39.15^{+0.85}_{-0.20}$ & $  3.98$ & $   3$ \\
NGC5457 & 14  3 21.60 & +54 19 45.02 & $  0.09^{+ 0.45}_{-0.08}$ & $ 1.17^{+1.13}_{-0.46}$ & $38.98^{+0.20}_{-0.09}$ & $  0.23$ & $   1$ \\
NGC5775 & 14 54 13.24 & + 3 32 44.89 & $  0.00^{+ 0.03}_{-0.00}$ & $ 1.34^{+0.49}_{-0.27}$ & $39.69^{+0.12}_{-0.07}$ & $ 12.32$ & $   6$ \\
NGC5775 & 14 54  0.97 & + 3 31 33.11 & $  0.48^{+ 1.32}_{-0.42}$ & $ 9.85^{+0.15}_{-8.01}$ & $40.66^{+0.09}_{-0.68}$ & $  2.64$ & $   2$ \\
NGC5775 & 14 54  0.96 & + 3 31 29.39 & $  0.61^{+ 1.21}_{-0.53}$ & $ 2.06^{+7.94}_{-0.89}$ & $39.82^{+0.67}_{-0.14}$ & $  0.70$ & $   3$ \\
NGC5775 & 14 53 59.45 & + 3 31 57.25 & $  0.24^{+ 0.20}_{-0.19}$ & $ 2.50^{+3.72}_{-0.85}$ & $40.19^{+0.40}_{-0.13}$ & $ 11.77$ & $  10$ \\
NGC5775 & 14 53 58.90 & + 3 32 16.78 & $  2.05^{+ 0.20}_{-0.18}$ & $ 1.97^{+0.29}_{-0.22}$ & $41.11^{+0.02}_{-0.02}$ & $ 55.83$ & $  57$ \\
NGC5775 & 14 53 56.80 & + 3 31 29.41 & $  0.14^{+ 0.28}_{-0.13}$ & $ 0.91^{+0.45}_{-0.26}$ & $39.37^{+0.17}_{-0.08}$ & $  7.23$ & $   3$ \\
NGC5775 & 14 53 55.92 & + 3 34  0.74 & $  0.00^{+ 0.07}_{-0.00}$ & $ 1.93^{+0.86}_{-0.46}$ & $39.97^{+0.17}_{-0.10}$ & $  8.57$ & $  11$ \\
NGC5775 & 14 53 55.76 & + 3 33 28.02 & $  2.05^{+ 0.90}_{-0.75}$ & $ 1.68^{+1.01}_{-0.47}$ & $40.28^{+0.09}_{-0.07}$ & $  8.66$ & $   7$ \\
NGC5775 & 14 53 55.25 & + 3 32 29.18 & $  0.08^{+ 0.24}_{-0.08}$ & $ 0.91^{+1.14}_{-0.35}$ & $39.49^{+0.25}_{-0.08}$ & $  0.59$ & $   3$ \\
NGC5775 & 14 53 54.75 & + 3 33 40.76 & $  0.47^{+ 1.07}_{-0.47}$ & $ 0.58^{+9.42}_{-0.31}$ & $39.26^{+0.99}_{-0.29}$ & $  0.70$ & $   1$ \\
NGC5775 & 14 53 53.71 & + 3 36 24.09 & $  0.00^{+ 0.32}_{-0.00}$ & $ 1.21^{+1.20}_{-0.44}$ & $39.34^{+0.25}_{-0.08}$ & $  4.62$ & $   1$ \\
NGC5775 & 14 53 53.14 & + 3 32 55.54 & $  0.01^{+ 1.61}_{-0.00}$ & $ 4.09^{+5.91}_{-2.95}$ & $39.87^{+0.54}_{-0.34}$ & $  6.18$ & $   3$ \\
NGC5775 & 14 53 48.29 & + 3 34  2.46 & $  0.44^{+ 0.72}_{-0.39}$ & $ 0.89^{+3.27}_{-0.37}$ & $39.52^{+0.44}_{-0.16}$ & $  1.77$ & $   1$ \\
NGC5775 & 14 53 44.70 & + 3 33 30.89 & $  0.00^{+ 0.01}_{-0.00}$ & $ 0.79^{+0.08}_{-0.05}$ & $40.14^{+0.02}_{-0.01}$ & $ 69.46$ & $  32$ \\
NGC5775 & 14 53 55.94 & + 3 29 12.83 & $  0.00^{+ 0.17}_{-0.00}$ & $ 0.99^{+0.75}_{-0.36}$ & $39.34^{+0.21}_{-0.04}$ & $  4.79$ & $   2$ \\
NGC6946 & 20 35  0.96 & +60 10 11.02 & $  0.21^{+ 0.10}_{-0.11}$ & $ 1.43^{+0.38}_{-0.22}$ & $38.73^{+0.07}_{-0.04}$ & $ 19.69$ & $  15$ \\
NGC6946 & 20 35  0.13 & +60  9  7.97 & $  0.22^{+ 0.03}_{-0.03}$ & $ 0.32^{+0.02}_{-0.03}$ & $39.46^{+0.08}_{-0.06}$ & $162.24$ & $  63$ \\
NGC6946 & 20 34 57.73 & +60  9 48.83 & $  0.27^{+ 0.11}_{-0.12}$ & $ 0.87^{+0.23}_{-0.15}$ & $38.65^{+0.05}_{-0.05}$ & $ 13.57$ & $  13$ \\
NGC6946 & 20 34 56.49 & +60  8 34.04 & $  0.29^{+ 0.23}_{-0.16}$ & $ 1.75^{+0.82}_{-0.43}$ & $38.84^{+0.13}_{-0.07}$ & $ 33.36$ & $  14$ \\
NGC6946 & 20 34 48.78 & +60  5 54.50 & $  0.17^{+ 0.18}_{-0.17}$ & $ 0.22^{+0.12}_{-0.06}$ & $38.88^{+0.58}_{-0.47}$ & $ 64.08$ & $  11$ \\
NGC6946 & 20 34 48.44 & +60  8 11.38 & $  0.03^{+ 0.20}_{-0.03}$ & $ 1.36^{+0.60}_{-0.37}$ & $38.35^{+0.14}_{-0.06}$ & $ 13.20$ & $   6$ \\
NGC6946 & 20 34 39.77 & +60  8 22.87 & $  3.71^{+ 4.66}_{-3.65}$ & $ 0.63^{+2.07}_{-0.28}$ & $38.69^{+1.34}_{-0.70}$ & $  1.07$ & $   1$ \\
NGC6946 & 20 34 36.48 & +60  9 30.46 & $  0.13^{+ 0.06}_{-0.03}$ & $ 0.38^{+0.04}_{-0.04}$ & $38.94^{+0.11}_{-0.06}$ & $ 72.85$ & $  31$ \\
NGC6946 & 20 34 34.42 & +60 10 33.08 & $  0.00^{+ 0.22}_{-0.00}$ & $ 0.52^{+0.13}_{-0.16}$ & $37.86^{+0.27}_{-0.01}$ & $  5.15$ & $   3$ \\
NGC6946 & 20 34 26.08 & +60  9  9.41 & $  0.14^{+ 0.04}_{-0.05}$ & $ 1.14^{+0.14}_{-0.12}$ & $38.97^{+0.02}_{-0.02}$ & $ 44.54$ & $  35$ \\
NGC6946 & 20 34 24.94 & +60  9  6.10 & $  0.00^{+ 0.09}_{-0.00}$ & $ 1.75^{+0.98}_{-0.47}$ & $38.37^{+0.19}_{-0.11}$ & $ 18.80$ & $   5$ \\
NGC6946 & 20 34 19.02 & +60 10  7.97 & $  0.00^{+ 0.75}_{-0.00}$ & $ 1.58^{+8.42}_{-1.15}$ & $37.90^{+1.05}_{-0.24}$ & $  0.32$ & $   1$ \\
NGC6946 & 20 35  5.32 & +60  6 23.10 & $  0.00^{+ 0.58}_{-0.00}$ & $ 1.92^{+2.13}_{-0.81}$ & $38.14^{+0.31}_{-0.11}$ & $  7.21$ & $   2$ \\
NGC6946 & 20 35  1.96 & +60 10  3.62 & $  0.12^{+ 0.24}_{-0.12}$ & $ 1.93^{+8.07}_{-0.78}$ & $38.41^{+0.79}_{-0.14}$ & $  1.95$ & $   4$ \\
NGC6946 & 20 34 24.71 & +60 10 38.83 & $  1.19^{+ 3.05}_{-1.01}$ & $ 9.83^{+0.17}_{-8.35}$ & $39.02^{+0.11}_{-0.65}$ & $  1.86$ & $   2$ \\
\enddata
\tablecomments{Host galaxy name; Right Ascension; Declination; $n_H$, equivalent hydrogen column density; $kT_{in}$, inner disk temperature; L, Bolometric X-ray luminosity; C-statistics; degree of freedom. }
\end{deluxetable}

